LLMBoost: Make Large Language Models Stronger with Boosting

Ensemble learning of LLMs has emerged as a promising alternative to enhance performance, but existing approaches typically treat models as black boxes, combining the inputs or final outputs while overlooking the rich internal representations and interactions across models.In this work, we introduce LLMBoost, a novel ensemble fine-tuning framework that breaks this barrier by explicitly leveraging intermediate states of LLMs. Inspired by the boosting paradigm, LLMBoost incorporates three key innovations. First, a cross-model attention mechanism enables successor models to access and fuse hidden states from predecessors, facilitating hierarchical error correction and knowledge transfer. Second, a chain training paradigm progressively fine-tunes connected models with an error-suppression objective, ensuring that each model rectifies the mispredictions of its predecessor with minimal additional computation. Third, a near-parallel inference paradigm design pipelines hidden states across models layer by layer, achieving inference efficiency approaching single-model decoding. We further establish the theoretical foundations of LLMBoost, proving that sequential integration guarantees monotonic improvements under bounded correction assumptions. Extensive experiments on commonsense reasoning and arithmetic reasoning tasks demonstrate that LLMBoost consistently boosts accuracy while reducing inference latency.

==> content/0_abstract.tex <==
\begin{abstract}





Ensemble learning of LLMs has emerged as a promising alternative to enhance performance, but existing approaches typically treat models as black boxes, combining the inputs or final outputs while overlooking the rich internal representations and interactions across models.Ensemble learning of LLMs has emerged as a promising alternative to enhance performance, but existing approaches typically treat models as black boxes, combining the inputs or final outputs while overlooking the rich internal representations and interactions across models.
In this work, we introduce \modelname, a novel ensemble fine-tuning framework that breaks this barrier by explicitly leveraging intermediate states of LLMs. Inspired by the boosting paradigm, \modelname incorporates three key innovations. First, a \textit{cross-model attention mechanism} enables successor models to access and fuse hidden states from predecessors, facilitating hierarchical error correction and knowledge transfer. Second, a \textit{chain training paradigm} progressively fine-tunes connected models with an error-suppression objective, ensuring that each model rectifies the mispredictions of its predecessor with minimal additional computation. Third, a \textit{near-parallel inference paradigm} pipelines hidden states across models layer by layer, achieving inference efficiency approaching single-model decoding.
We further establish the theoretical foundations of \modelname, proving that sequential integration guarantees monotonic improvements under bounded correction assumptions. Extensive experiments on commonsense reasoning and arithmetic reasoning tasks demonstrate that \modelname consistently boosts accuracy while reducing inference latency.



% Ensemble learning is widely recognized as an effective way to improve model performance, and recent research has increasingly focused on its application to large language models (LLMs). Existing studies on LLM ensemble learning primarily concentrate on token-level aggregation or adjustments of the training data, often overlooking the errors and reasoning processes inherent in model outputs. To address this gap, we propose \textsc{LLMBoost}, a boosting-based ensemble framework for LLMs that incrementally corrects reasoning errors committed by the immediately preceding model in the ensemble sequence. Instead of focusing on individual tokens, LLMBoost performs ensemble learning on LLMs’ reasoning trajectories; it further introduces an error-aware loss function to encourage models to explicitly rectify earlier mistakes during training. Additionally, unlike prior ensemble methods that rely on sequential execution, we design a hierarchy-aware pipelined parallel inference strategy to significantly accelerate inference. Extensive experiments across multiple benchmarks demonstrate that \textsc{LLMBoost} achieves substantial performance gains over existing approaches. Moreover, comprehensive evaluations conducted in real-world cloud environments at \dianxinlab Lab confirm the effectiveness and practicality of our method.


% 集成学习是一种能够快速提升模型性能的方法，近期有很多研究开始聚焦在大模型集成学习上。现有的大模型集成学习往往是集中在token级的集成，亦或是在训练数据上进行调整，然后这些方法往往忽略xxxx。基于此，我们提出了llmboost，一种基于boosting 逐步修正思想的大模型集成学习方式。我们的方法会从大模型的推理轨迹上进行集成，此外我们还提出了错误感知损失函数，可以帮助大模型在训练过程中，更好的去修正前一个模型犯下的错误。并且现有的大模型集成学习都是线性的执行顺序，我们针对我们的方法提出了层级感知并行推理方法，提高推理速度。在多个基准测试上的广泛实验表明，llmboost相较于现有方法能够显著提升性能，并且我们的方法在天翼云实验室进行了更深入的测试，并且取得了很好的效果。
\end{abstract}

==> content/1_introduction.tex <==
\section{Introduction}


%\ban{Add citations for the following @zehao}
Large Language Models (LLMs) have revolutionized natural language processing, building on the Transformer’s attention mechanism Large Language Models (LLMs) have revolutionized natural language processing, building on the Transformer’s attention mechanism \citep{vaswani2017attention}. Individual models such as GPT-4 . Individual models such as GPT-4 \citep{achiam2023gpt}, Llama-3 , Llama-3 \citep{touvron2023llama}, and Qwen , and Qwen \citep{yang2025qwen3} have demonstrated remarkable performance across a wide range of domains. have demonstrated remarkable performance across a wide range of domains.
 Meanwhile, ensemble learning of LLMs — combining multiple agents to yield stronger, more robust performance — is gaining attention \citep{chen2025harnessing, lu2024merge}. However, despite its promise, the exploration of ensembles in the LLM era remains relatively nascent.

%Nevertheless, training LLMs requires massive computational resources that remain beyond the reach of most institutions. Instead of pushing toward ever-larger individual models, ensemble learning of pretrained LLMs \citep{chen2025harnessing,lu2024merge} has emerged as a promising alternative for building stronger systems, yet this direction remains underexplored.


Most existing LLM ensemble methods treat each model as a black box and fuse only their final outputs—either at the token level or the full-response level \citep{chen2025harnessing}—via majority voting \citep{li2024more,yu2024breaking}, weighted aggregation \citep{li2024purifying}, or routing strategies \citep{shnitzer2023llm}. However, these approaches ignore the rich information embedded in the hidden representations of the LLMs, and more fine-grained interactions—beyond mere output fusion—are needed to fully exploit complementary knowledge across models.

In this paper, we go beyond conventional output-level ensembling and propose a novel fine-tuning framework for LLM ensembles, \modelname, which enables fine-grained internal interactions by progressively leveraging the hidden representations within each model in the boosting style. Our main contributions are summarized as follows.

%Inspired by the “boosting” paradigm, \modelname extracts and leverages the internal states of LLMs during ensemble learning, progressively fine-tuning each model to complement the under-learned knowledge of its predecessors.


[\textbf{Model Architecture}]. We design a residual cross-model attention mechanism in which successor models can adaptively access and fuse the intermediate hidden states of predecessor models, rather than relying solely on its final outputs. The cross-model attention is constructed at the layer level, breaking the black-box barrier and enabling state-driven hierarchical interaction among LLMs. In addition, progressively targeted fusion is applied to output logits, which allows \modelname to transfer valid knowledge across models effectively.


[\textbf{Chain Training}]. We introduce a sequential training framework for connected LLMs,
%, where a backbone model is trained with LoRA adapters to preserve general knowledge from pretraining, 
and each subsequent model is fine-tuned based on the training log of its predecessor. Inspired by the boosting paradigm, the role of a successor model is to rectify the key tokens of its predecessor. Thus, we propose an error-suppression objective, which suppresses the maximal (incorrect) logit produced by the predecessor while enhancing the correct one. By doing so, \modelname significantly reduces the overall computational requirement while ensuring that performance is progressively boosted across the chain of models.



[\textbf{Near-Parallel Inference}].
We propose a near-parallel streaming inference paradigm to minimize the latency introduced by sequential interactions among LLMs. Instead of waiting for the predecessor to complete full sequence generation, \modelname transmits hidden states at the layer level without delay: 
the hidden state from the $(l-1)$-th layer of the predecessor is immediately passed to the $l$-th layer of the successor for parallel computation, even before the forward pass is completed. 
This pipelined design significantly reduces inference latency, achieving performance close to that of a single model while substantially outperforming vanilla inference ensembles.


[\textbf{Theoretical Analysis}].
We provide a formal theoretical analysis for \modelname, establishing a principled foundation for its sequential error-correction mechanism. We prove that, under the condition that each new model effectively corrects its predecessor's errors, the ensemble's performance is guaranteed to improve with each model added. This guarantee holds when the contribution of each new model is appropriately weighted, demonstrating a clear theoretical path toward progressively enhancing prediction accuracy through our boosting-style integration. Our analysis is grounded in Mean Squared Error, offering a direct and comprehensive measure of performance gains.

[\textbf{Empirical Performance}] .
Extensive experiments on commonsense and arithmetic reasoning tasks — including a custom set co-developed with \dianxinlab — confirm our approach’s effectiveness. Compared to other ensemble baselines, \modelname consistently enhances performance across tasks in tests: it delivers an overall average improvement of 3.9\%, with an even larger 6.6\% as the maximum improvement, with 3\% improvement observed specifically on \dianxindataset(\dianxindatasetshort). Moreover, our near-parallel decoding strategy reduces inference latency by 47\% compared to conventional sequential ensembles, demonstrating clear advantages in efficiency.





%This design fundamentally departs from existing methods by exploiting internal representations rather than relying solely on external ensemble mechanisms, enabling more effective error reduction and knowledge integration.





%To address the above limitations, we propose \modelname—a dedicated LLM ensemble framework that enables "white-box" interaction and efficient inference. Its core innovations target the two key flaws of existing methods:


%we leverage hidden state-driven fine-grained interaction to break the black-box barrier. We design a residual cross-attention mechanism that allows subsequent models to adaptively access and fuse the intermediate hidden states of predecessor models instead of only using final outputs. Since LLM hidden states encode hierarchical information,  \modelname can precisely locate and correct errors at specific layers and transfer valid knowledge across models.






%Instead of waiting for full sequence generation of, \modelname passes hidden states between models at the layer level: the l-th layer hidden state of the preceding model is immediately transmitted to the l-th layer of the subsequent model for parallel computation. This pipeline design reduces inference latency to only 10–20\% higher than a single model—far below the 200–300\% increase of traditional ensembles.






%The primary contributions of this work are fourfold:

%A novel Boosting-inspired ensemble framework for LLMs: We propose a hierarchical ensemble architecture where a base model generates initial outputs/hidden states, and supervisor models iteratively refine them via hidden state interaction. This adapts traditional boosting to autoregressive LLMs, transforming "sample-level refinement" into "hidden state-level boosting."

%Low-latency parallel streaming inference: We design a layer-wise parallel pipeline that transmits hidden states between models in real time, resolving the latency bottleneck of sequential ensemble methods. This enables BoostingLLM to maintain efficiency while improving performance.







%master diverse tasks—from text classification to advanced reasoning—via trillion-scale pre-training and fine-tuning, achieving human-level performance on GSM8K\cite{cobbe2021training} and SMAVP\cite{patel2021nlp}.




%Yet single LLMs face critical flaws: they suffer from hallucinations and inconsistent reasoning\cite{kalai2024calibrated}; different LLMs exhibit striking disparities in their specialized domains\cite{jiang2023llm}, LLM ensemble learning addresses these issues by combining smaller or domain-specialized LLMs to harness their complementary strengths, achieving synergistic performance gains with greater practicality\cite{chen2025harnessing}.However, existing methods still fail to fully exploit small-model potential, leaving gaps in interaction and efficiency.



%These ensemble approaches—both traditional adaptations \cite{}\cite{} and LLM-specific variants \cite{}\cite{}—face two critical flaws limiting practicality. 



%Most methods treat LLMs as independent black boxes, fusing only final outputs \cite{yao2024determine}\cite{li2024more} without leveraging internal information: vote-based ensembles of models, for instance, only aggregate token-level outputs and cannot exploit one model’s intermediate reasoning to guide others. This overlooks the fact that LLM hidden states at different layers are known to encode rich hierarchical information \cite{azaria2023internal}, thereby wasting valuable opportunities for error correction and knowledge transfer embedded in these representations. Additionally, existing ensembles rely on sequential execution or parallel but independent generation, resulting in several times higher latency than single models \cite{zhang2023ecoassistant}, leading to higher real-time application latency.

==> content/2_relatedwork.tex <==
  % \vspace{-10pt}

\section{Related Work}
  % \vspace{-10pt}

% LLM ensemble methods fall into two primary categories: one categorized by integration timing relative to reasoning, and the other categorized by operational target—whether they operate on models’ final outputs or intermediate states during reasoning. By integration timing relative to reasoning, they include pre-inference methods that focus on task-model matching via Pretrained routing as in \cite{ong2024routellm}\cite{shnitzer2023llm} and Non-pretrained routing as in \cite{sikeridis2025pickllm}\cite{zhang2025avengers}; inference-time methods that enable dynamic fusion during decoding such as token-level probability aggregation \cite{yao2024determine}\cite{yu2024breaking}\cite{xu2024bridging}\cite{li2024purifying} and span-level segment integration \cite{xu2024hit}\cite{fu2025rlae}; and post-inference methods that fuse complete outputs through non-cascaded approaches \cite{li2024more}\cite{guha2024smoothie} and cascaded strategies such as difficulty-aware revision \cite{yue2023large}. By operational target, they split into model-level approaches that operate on final outputs including majority voting \cite{li2024more}, weighted fusion \cite{guha2024smoothie}, and routing-based selection methods like Routellm \cite{ong2024routellm} and PickLLM \cite{sikeridis2025pickllm}, and internal-model approaches that intervene in reasoning processes.
% \cite{he2024llm} proposes a diverse prompt–based LLM ensemble method, with demonstrated applications in data imputation.
% Internal-model methods remain relatively underexplored, with few leveraging intermediate hidden states for fine-grained interaction. Our work advances internal-model approaches with a token-level dynamic correction framework rooted in boosting; it enables subsequent models to access and fuse predecessors’ intermediate hidden states—not just final outputs—for precise error correction, addressing the gap of insufficient intermediate interaction in existing methods while ensuring stable performance gains.



%operate only on final outputs, including majority voting \cite{li2024more}, weighted fusion \cite{guha2024smoothie}, and routing-based selection such as Routellm \cite{ong2024routellm} and PickLLM \cite{sikeridis2025pickllm}; and Prompt-based ensemble 



\textbf{LLM Ensemble Methods}.
Existing LLM ensemble methods primarily focus on output fusion using various strategies.
First, inference-time methods enable dynamic integration during decoding, such as token-level probability aggregation \citep{yao2024determine,yu2024breaking,xu2024bridging,li2024purifying} and span-level integration \citep{xu2024hit,fu2025rlae}. Other methods operate on the final outputs through majority voting \citep{li2024more}, weighted fusion \citep{guha2024smoothie}, routing-based selection \citep{ong2024routellm,sikeridis2025pickllm}, and prompt-based ensembles \citep{he2024llm}.
Second, post-inference methods fuse complete outputs, either via non-cascaded aggregation \citep{li2024more,guha2024smoothie} or cascaded strategies such as difficulty-aware revision \citep{yue2023large}.
Third, pre-inference methods focus on task–model matching, including pretrained routing \citep{ong2024routellm,shnitzer2023llm} and non-pretrained routing \citep{sikeridis2025pickllm,zhang2025avengers}.
While effective, these approaches treat models largely as independent black boxes, overlooking the internal representations and cross-model interactions that could further enhance ensemble performance.


\textbf{Boosting Methods.}
Boosting \citep{friedman2001greedy,hastie2009elements,ke2017lightgbm} is a classical ensemble paradigm that builds strong learners by sequentially correcting the errors of prior learners. Gradient Boosting minimizes loss by fitting new learners to the residuals of previous outputs \citep{hastie2009elements,chen2016xgboost}, while AdaBoost reweights samples to emphasize misclassified instances and combines learners via weighted voting \citep{freund1997decision,li2008adaboost}. Recent work has extended boosting to LLMs: \cite{agrawal2025ensemw2s} applied AdaBoost to train a series of weak LLMs into a stronger model\footnote{We did not find open-source code, and thus we exclude it from experimental comparisons.}, but this approach ensembles over training samples while still ignoring internal interactions among LLMs. \cite{zou2025transformer} introduced copilot adapters to correct errors during model fine-tuning, but the scope is limited to a single auxiliary adapter.



Distinct from existing LLM ensemble works, our work advances the field by ensembling on internal representations. \modelname enables subsequent models to access and fuse predecessors’ intermediate hidden states—not just final outputs—for precise error correction, addressing the gap of insufficient intermediate interaction in existing methods while ensuring stable performance gains.





%Internal-model methods remain relatively underexplored, with few leveraging intermediate hidden states for fine-grained interaction. Our work advances internal-model approaches with a token-level dynamic correction framework rooted in boosting; it enables subsequent models to access and fuse predecessors’ intermediate hidden states—not just final outputs—for precise error correction, addressing the gap of insufficient intermediate interaction in existing methods while ensuring stable performance gains.






%Gradient Boosting applies gradient descent to minimize loss, with each new learner fitting residuals of previous ensemble outputs \cite{friedman2001greedy}\cite{friedman2002stochastic}\cite{hastie2009elements}. XGBoost optimizes this with regularization and parallel processing \cite{chen2016xgboost}, while LightGBM boosts efficiency via histogram-based splitting and GPU acceleration \cite{ke2017lightgbm}, collectively enhancing predictive performance in supervised learning.


%\ban{To do: add EnsembleW2S, add T-Copilot}

==> content/3_methods.tex <==

\section{Proposed Framework: \modelname}
\label{method}

\begin{figure*}[!t]
% \captionsetup{font=footnotesize}
  \centering
  % \vspace{-0.05in}
  \includegraphics[width= 1.0 \textwidth]{iclr2026/pictures/model_architecture.png}
  \caption{\modelname Framework. The overall framework comprises three key components: (1) \modelname Model Design, (2) Training Paradigm, and (3) Error-Suppression Objective.}
  \label{fig:overall_framework}
  \vspace{-10pt}
\end{figure*}

We introduce \modelname, a hierarchical ensemble fine-tuning framework that enables LLMs to perform internal interactions during both training and inference. In the following sections, we elaborate on \modelname from three perspectives: its architecture, training paradigm, and inference paradigm.

%Our approach is inspired by the core idea of XGBoost \cite{chen2016xgboost}—progressive refinement—but breaks away from its classical formulation through a series of systematic modifications. Specifically, we transform the traditional residual correction into \textbf{fine-grained token-level refinement}, and optimize the original serial dependency into a \textbf{hierarchy-aware pipelined parallelism}. In addition, we design an \textbf{error-aware loss function} that, while preserving the standard cross-entropy supervision, imposes extra constraints on tokens mispredicted by the previous model, thereby enabling more targeted optimization. This design not only enhances robustness but also improves inference efficiency. \\

\textbf{Notations}. As illustrated in Figure~\ref{fig:overall_framework}, \modelname is designed as a sequential ensemble of pretrained LLMs, where each LLM adopts a decoder-only Transformer architecture. Suppose there are $(1+n)$ LLMs in total. Formally, the ensemble can be represented as
$\mathcal{M} = \{ m_0(\cdot; \theta_0), m_1(\cdot; \theta_1), \dots, m_n(\cdot; \theta_n) \}$,
where we use $m_i \in \mathcal{M}$ to denote the $i$-th model and $\theta_i$ its trainable parameters for simplicity.
In one fine-tuning round $\tau$, we sample an input–output pair $(X_\tau, Y_\tau)$ from a data distribution $D_{\mathcal{X}, \mathcal{Y}}$, where $X_\tau$ is the input sequence and $Y_\tau$ the corresponding target sequence. \modelname generates the output sequence $\widehat{Y}_\tau$ in an autoregressive manner, aiming to approximate the target sequence $Y_\tau$. 
At the $t$-th decoding step, let $z^{(i)}_t$ denote the logits produced by the $i$-th model, and let $p^{(i)}_t = \mathrm{softmax}(z^{(i)}_t)$ be the corresponding probability distribution over the vocabulary. 
The predicted token of the $i$-th model is then
$\hat{y}^{(i)}_t = \arg\max p^{(i)}_t,$
while the ground-truth token is denoted by $y^{\ast}_t$.



\subsection{Framework Architecture}
%Our proposed \textbf{\modelname} framework is built upon decoder-only Transformer architectures, with model parameters initialized from publicly available HuggingFace checkpoints.

%In the following sections, we will elaborate on the model design, the training paradigm, and the inference paradigm, respectively.





% \iffalse

% \begin{wrapfigure}{r}{0.45\textwidth} % r=右侧，宽度自调
%   \centering
%   \vspace{1em}
%   \includegraphics[width=0.43\textwidth]{iclr2026/pictures/modeldesign& trainingParadigm.png}
%   \caption{\modelname Framework. The overall framework comprises two key components: \textbf{(1) \modelname Model Design}, \textbf{(2) Training Paradigm}, and \textbf{ Inference Paradigm} (details are provided in Fig.~\ref{fig:inference}).}
%   \label{fig:overall_framework}
% \end{wrapfigure}
% \fi
%Each sub-model in \modelname is initialized from public pre-trained checkpoints, while lightweight modules are newly introduced to support task adaptation and cross-model interaction. 
%Formally, the ensemble can be represented as:
%$\mathcal{M} = \{ m_0(\cdot; \theta_0), m_1(\cdot; \theta_1), \dots, m_K(\cdot; \theta_k) \}$,
%where $m_i$ denotes the $i$-th model and $\theta_i$ its trainable parameters. For simplicity, we use $m_i$ to denote $m_i(\cdot;\theta_i)$ in the following.




%\subsubsection{Fine-grained Token-level Refinement}
\paragraph{Cross-Model Attention.}
A key innovation of \modelname lies in its fine-grained token-level refinement mechanism.
Unlike conventional ensembles where models operate independently, each model $m_i$ directly accesses and fuses the hidden representations of its predecessor $m_{i-1}$, thereby enabling hierarchical interaction across the $n$ LLMs.
Concretely, at the $t$-th decoding step, let $h^{(i-1)}_{l-1,t}$ denote the hidden state from the $(l-1)$-th Transformer layer of the $(i-1)$-th model. The cross-model attention mechanism at the $l$-th layer of the $i$-th model is defined as:
\begin{equation}
\label{equ:hiddenStatesAddNorm}
    \tilde{h}^{(i)}_{l,t} = 
\begin{cases}
\mathrm{LayerNorm}\!\big(h^{(i)}_{l-1,t} + h^{(i-1)}_{l-1,t}\big), & \text{if} \ l \bmod \eta = 0, \\[6pt]
h^{(i)}_{l-1,t}, & \text{otherwise}.
\end{cases}
\end{equation}
where $\eta$ is an integer constant that controls the sparsity of cross-model connections among the $n$ LLMs.
With the enhanced hidden states, the cross-attention output is calculated by:

\begin{equation}
   \hat{h}^{(i)}_{l,t} 
= \mathrm{softmax}\!\Big(\tfrac{Q^{(i)}_{l,t} (K^{(i)}_{l,t})^\top}{\sqrt{d_k}}\Big) V^{(i)}_{l,t}, \ \ \text{where} \ Q^{(i)}_{l,t} = \tilde{h}^{(i)}_{l,t} W_Q, 
\quad K^{(i)}_{l,t} = \tilde{h}^{(i)}_{l,t} W_K, 
\quad V^{(i)}_{l,t} = \tilde{h}^{(i)}_{l,t} W_V,
\end{equation}
followed by another residual enhancement:
\begin{equation}
h^{(i)}_{l,t} = \mathrm{LayerNorm}\!\big( \hat{h}^{(i)}_{l,t}+ \tilde{h}^{(i)}_{l,t} \big).
\end{equation}

This design equips later models with structured access to their predecessors’ reasoning process, yielding:
 \emph{error correction}, where inaccurate states are adjusted, and 
 \emph{knowledge reinforcement}, where correct signals are amplified.  

For the input and output streaming, the input sequence $X_\tau$ is shared across all models in \modelname, while the output fusion streaming incorporates two key innovations.

(1) \textbf{Error-Token Forward Pass}. 
To enable successor models to recognize and correct token-level errors made by their predecessors, we introduce an error-token forwarding mechanism. This design improves both performance and robustness of \modelname. During training, the error logits produced by model $m_i$ are sequentially passed to its successor $m_{i+1}$ under a specific learning objective (detailed in the next section).
At the $t$-th decoding step, let $\hat{y}^{(i)}_t = \arg\max p^{(i)}_t$ denote the predicted token index, where the error tokens are defined as follows:
\begin{equation}
\text{ErrorToken}^{(i)}_t =
\begin{cases}
\hat{y}^{(i)}_t, & \text{if } \hat{y}^{(i)}_t \neq y_t^{\ast}, \\[6pt]
\emptyset, & \text{otherwise},
\end{cases}
\end{equation}
where $y_t^{\ast}$ denotes the ground-truth token. Thus, only incorrect token indices are passed forward, encouraging successors to explicitly learn from predecessor mistakes.



(2) \textbf{Key-Logits Backward Pass}.
To further stabilize the inference process, we propose a top-$k$ logits fusion strategy, where later successor models pass key logits backward to the base model $m_0$.  
Instead of aggregating over the entire vocabulary, each sub-model contributes only its most informative token logits, thereby reducing the influence of noisy, low-confidence outputs.  
Formally, given the logit distribution $z_t^{(i)}$ from the $i$-th model $m_i$, we define the restricted candidate set and the ensemble update rule as:
\begin{equation} 
\label{equ:logitsFusion}
\begin{aligned} 
z_t &= z^{(0)}_t + \sum_{i=1}^{n} \lambda_i \cdot \mathrm{Mask}(z^{(i)}_t, \mathcal{V}_{\text{top-}k}^{(i)}), \ \ \text{where} \ \mathcal{V}_{\text{top-}k}^{(i)} = \mathrm{\arg \text{top-k}}(z^{(i)}_t),  
\end{aligned} 
\end{equation} 
where $z_t$ denotes the final raw logits, $\lambda_i$ is a scaling coefficient, and is a scaling coefficient, and $\mathrm{Mask}(\cdot)$ restricts contributions to the top- restricts contributions to the top-$k$ candidates by setting all other indices to zero in each logit distribution. candidates by setting all other indices to zero in each logit distribution.


% By filtering out tokens with negligbible probability mass, this mechanism (i) \emph{suppresses spurious predictions} and (ii) \emph{promotes model agreement} by concentrating fusion on a shared subset of plausible candidates.  
% Together with parallel streaming, this ensures both efficiency and robustness in multi-model inference.  

\iffalse
\textbf{To some extent, To some extent, \modelname can be regarded as a more fine-grained ensemble model. Unlike many approaches that only perform ensembling at the token level,  can be regarded as a more fine-grained ensemble model. Unlike many approaches that only perform ensembling at the token level, \modelname realizes cross-model integration within the internal representations and reasoning process, thereby establishing a mechanism of progressive correction and reinforcement along the generation path. realizes cross-model integration within the internal representations and reasoning process, thereby establishing a mechanism of progressive correction and reinforcement along the generation path.}
\fi



% For $i \geq 1$, each subsequent model $m_i$ is a \emph{boosting supervisor} that conditions on the internal representations of its predecessor rather than decoding in isolation. When the inherited states are erroneous or unstable, $m_i$ corrects the trajectory; when they are reliable, $m_i$ amplifies and stabilizes them. 
% This induces a progressive correction chain in which $m_0$ proposes an initial decoding path, $m_1$ audits and refines it, and the process iterates through $m_2,\ldots,m_k$. 

%An overview of our framework is illustrated in Figure~\ref{fig:overall_framework}.The first model $m_0$ serves as the \emph{base generator}, performing standard autoregressive decoding over the vocabulary $\mathcal{V}$. It produces both token logits and intermediate hidden states during the forward process.
%For $i \geq 1$, each subsequent model $m_i$ is a \emph{boosting supervisor} that conditions on the internal representations of its predecessor rather than decoding in isolation. When the inherited states are erroneous or unstable, $m_i$ corrects the trajectory; when they are reliable, $m_i$ amplifies and stabilizes them. 
%This induces a progressive correction chain in which $m_0$ proposes an initial decoding path, $m_1$ audits and refines it, and the process iterates through $m_2,\ldots,m_k$. 
%At each stage, the model conditions on its predecessor’s signals and either rectifies deviations or strengthens correct cues, yielding a final output that reflects $k$ rounds of structured, cross-model supervision.


\subsection{Chain Training Paradigm}
\textbf{Error-Suppression Objective.}
To enable each model to refine its predecessor by correcting erroneous predictions while preserving correct ones, we introduce a token-level suppression loss.  
The principle is that each $m_i$ should preserve plausible predictions from $m_{i-1}$, while intervening 
only when necessary. Formally,  we define the error-suppression loss:
\begin{equation}
\label{equ:preference_optimization}
    \mathcal{L}_{s,t} = - \log\!\Big( \sigma\!\big( \beta \,[ \log p^{(i)}_t[y_t^{ \ast}] - \log p_t^{(i)}[\text{ErrorToken}^{(i-1)}_t]] \big) \Big) \cdot \mathbf{1}\!\{ \text{ErrorToken}^{(i-1)}_t\neq \emptyset \},
\end{equation}
where $\sigma$ is the sigmoid, $\beta$ a scaling factor, and the indicator $\mathbf{1}$ activates the loss only at positions where the predecessor $i-1$ predicts incorrectly.
The overall objective for $m_i$ becomes:
\begin{equation}
\label{equ:totalloss}
\mathcal{L}_i = \sum_t   \mathcal{L}_{s,t}    - \alpha\sum_t \log p^{(i)}_{t}[y_t^{ \ast}],
\end{equation}
where the right item is the cross-entropy loss, and $\alpha$ is a balance coefficient.  
This dual-objective strategy endows the ensemble with a \emph{correction-while-retaining} ability, 
preserving useful signals while refining erroneous ones.



\begin{algorithm}[htbp]
\caption{\modelname: Training Process}
\label{alg:chained_ensemble}
\SetAlgoLined
\LinesNumbered
% \KwIn{Base model list $\mathcal{M} = \{m_0(\cdot; \theta_0), m_1(\cdot; \theta_1), \dots, m_n(\cdot; \theta_n)\}$, training dataset $\mathcal{D}$, Log pool $g$}
% \KwOut{Fine-tuned model list $\mathcal{\tilde{M}}= \{\tilde{m}_0(\cdot; \theta_0), \tilde{m}_1(\cdot; \theta_1), \dots, \tilde{m}_n(\cdot; \theta_n)\}$}
\KwIn{Base model list $\mathcal{M} = \{m_0, m_1, \dots, m_n\}$, training dataset $\mathcal{D}$, }
\KwOut{Fine-tuned model list $\mathcal{\tilde{M}}= \{\tilde{m}_0, \tilde{m}_1, \dots, \tilde{m}_n\}$}
% \textbf{Stage 1: Train the base model $m_0(\cdot; \theta_0)$}\;
% Initialize $m_0(\cdot; \theta_0) \gets$ ApplyLoRA($m_0(\cdot; \theta_0)$, $\phi$)\;
Initialize log pool $g$ \;
\textbf{Stage 1: Train the base model $m_0$}\;
\For{each batch $(x, y^{\ast}) \in \mathcal{D}$}{
    % Forward pass: $z^{(0)} \gets m_0(x; \theta_0)$\;
    Forward pass: $z^{(0)} \gets m_0(x)$\;
    Compute Cross-Entropy loss:$\mathcal{L}_0 \gets \text{CrossEntropyLoss}(z_0, y^{\ast})$\;
    Update $m_0$ parameters via LoRA using $\mathcal{L}_0$\;
    % Fine-tune $m_0$ via LoRA using $\mathcal{L}_0$: $\tilde{m}_0 \gets m_0$\;
    % Update $m_0(\cdot; \theta_0)$ parameters via LoRA fine-tuning using $\mathcal{L}_0$\;
    % Record training log: $g \gets \text{UpdateLog}(g, m_0,\{h^{(0)}, \text{ErrorToken}^{(0)}\})$
}
Obtain fine-tuned model: $\tilde{m}_0 \gets m_0$\;
\textbf{Stage 2: Train subsequent models $\{m_1(\cdot; \theta_1), \dots, m_n(\cdot; \theta_n)\}$}\;
\For{$i = 1$ \KwTo $n$}{
    % Initialize $m_i(\cdot; \theta_i) \gets$ ApplyLoRA($m_i(\cdot; \theta_i)$, $\phi$)\;
    \For{each batch $(x, y^{\ast}) \in \mathcal{D}$}{
        Get previous model's inference trajectory: $\{h^{(i-1)},\text{ErrorToken}^{(i-1)}\} \gets \tilde{m}_{i-1}(x)$\;
        % Get hidden states $h^{(i-1)}$ and predicted tokens $z^{(i-1)}$ from $\tilde{m}_{i-1}(x)$\;
        % Get $m_{i-1}$ training log:  $\{h^{(i-1)}, \text{ErrorToken}^{(i-1)}\} \gets \text{ReadLog}(g, m_{i-1})$\;
        Forward pass: $z^{(i)} \gets m_i(x,h^{(i-1)})$\;
        Compute Error-Suppression loss $\mathcal{L}_i$ via \ref{equ:totalloss} using $\{ z^{(i)},y^{\ast},\text{ErrorToken}^{(i-1)}\}$\;
        Update $m_i$ parameters via LoRA using $\mathcal{L}_i$\;
        % Fine-tune $m_i$ via LoRA using $\mathcal{L}_i$: $\tilde{m}_i \gets m_i$\;
        % Update $m_i(\cdot; \theta_0)$ parameters via LoRA fine-tuning using $\mathcal{L}_i$\;
        % Record training log: $g \gets \text{UpdateLog}(g, m_i,\{h^{(i)}, \text{ErrorToken}^{(i)}\})$
    }
    Obtain fine-tuned model: $\tilde{m}_i \gets m_i$\;
}
\KwRet{$\{\tilde{m}_0(\cdot; \theta_0), \tilde{m}_1(\cdot; \theta_1), \dots, \tilde{m}_n(\cdot; \theta_n)\}$}
\end{algorithm}

\textbf{Training Pipeline}.
% To enable efficient adaptation of large ensembles, we adopt a \emph{two-stage, chained fine-tuning} strategy (Algorithm~\ref{alg:chained_ensemble}). This design ensures that each sub-model learns not only from ground-truth supervision but also from the reasoning trajectory of its predecessor.
Our model adopts a two-stage chained fine-tuning strategy (see Algorithm~\ref{alg:chained_ensemble}), which ensures that each sub-model learns not only from ground-truth supervision but also from the reasoning trajectory of its predecessor.
In the first stage, the base model $m_0$ is adapted to the target task following standard  is adapted to the target task following standard LoRA fine-tuning. The parameter updates of  fine-tuning. The parameter updates of $m_0$ are solely driven by the input data  are solely driven by the input data $x$ and the ground-truth labels  and the ground-truth labels $y^{\ast}$.
In the second stage, subsequent models $m_i $ are fine-tuned in a chained manner. Specifically, for each model, we first extract the internal hidden states $h^{(i-1)}$ and error tokens $\text{ErrorToken}^{(i-1)}$ from its predecessor $\tilde{m}_{i-1}$. The input $x$, together with $h^{(i-1)}$, is then fed into $m_i$ for training. The Error-Suppression loss is computed using $z^{(i)}$,  $y^{\ast}$, and $\text{ErrorToken}^{(i-1)}$. This mechanism enables later models to progressively correct the reasoning errors of earlier models, thereby improving the overall ensemble performance.

% \textit{Stage 1 (Base adaptation).}  
% A base model $m_0$ is first adapted to the target data using LoRA adapters. This stage equips $m_0$ with task-specific capabilities while preserving general knowledge from pretraining. 
%  Additionally, the predicted tokens and intermediate hidden states generated by $m_0$ will serve as training priors for subsequent models.

% \textit{Stage 2 (Chained Fine-tuning).}  
% Subsequent models $m_i \ (i \geq 1)$ are fine-tuned sequentially, each conditioned on its predecessor. 
% Given a training batch $(X,Y)$, we record all hidden states $h^{(i-1)}_{l-1,t}$ and error tokens $\text{ErrorToken}^{(i-1)}_t$ during the fine-tuning of $m_{i-1}$. These signals are then injected into $m_i$, which is trained with the error-suppression objective. This process is repeated iteratively across the ensemble, enabling later models to progressively refine and correct the reasoning of earlier ones.
%A forward pass through $m_i$ produces two complementary objectives: the cross-entropy loss $\mathcal{L}_i$ against the ground truth $y$, and a preference loss $\mathcal{L}_p$ that encourages alignment with $\tilde{x}$ whenever the predecessor’s predictions are plausible. The combination of these two objectives ensures that each model learns to refine its predecessor’s output while preserving useful intermediate information.



% \textit{Stage 1 (Base adaptation).}  
% A base model $m_0$ is first adapted to the target data using LoRA adapters, with the pretrained backbone parameters kept frozen. This stage equips $m_0$ with task-specific capabilities while preserving general knowledge from pretraining. Importantly, $m_0$ provides both predicted token sequences and intermediate hidden representations, which later serve as structured priors for downstream models.

% \textit{Stage 2 (Chained Fine-tune).}  
% Subsequent models $m_i \ (i \geq 1)$ are fine-tuned sequentially, each conditioned on the outputs of its predecessor. Given a training batch $(x,y)$, we first obtain the predicted tokens $\tilde{x}$ and hidden states $h_{i-1}$ from $\tilde{M}_{i-1}(x)$. These signals are then injected into $m_i$ by augmenting its input with the original sequence $x$, the previously generated tokens $\hat{y}_{i-1}$, and the hidden states $h_{i-1}$. A forward pass through $m_i$ produces two complementary objectives: the cross-entropy loss $\mathcal{L}_i$ against the ground truth $y$, and a preference loss $\mathcal{L}_p$ that encourages alignment with $\tilde{x}$ whenever the predecessor’s predictions are plausible. The combination of these two objectives ensures that each model learns to refine its predecessor’s output while preserving useful intermediate information.

\begin{figure*}[!th]
% \captionsetup{font=footnotesize}
  \centering
  \includegraphics[width= 0.8\textwidth]{iclr2026/pictures/InferenceParadigm_v3.png}
  \caption{\textbf{Near-parallel inference paradigm.} 
The figure uses the timeline as the axis to show the computation state of each model at each moment. Hidden states are propagated across layers and models, and logits are aggregated and decoded into the final prediction, enabling overlapped computation and reduced inference latency.}
  \label{fig:inference}
  \vspace{-10pt}
\end{figure*}

\subsection{Near-Parallel Inference Paradigm} 

As each successor model $m_i$ depends on the intermediate hidden states of its predecessor $m_{i-1}$, a naive decoding scheme requires $m_i$ to begin its decoding only after $m_{i-1}$ has completed the entire decoding process. This results in an inference time complexity of $O(n)$ if one model takes $O(1)$ time per sequence, which becomes impractical when $n$ is large.


To address this, we propose a near-parallel inference
% layer-wise parallel streaming
paradigm (Algorithm~\ref{alg:parallel_inference_simple} in Appendix \ref{app:Near_Parallel_Algorithm}), which enables efficient inference across multiple models. Instead of waiting for the predecessor to finish full sequence generation, \modelname streams hidden states at the \emph{layer level}: the hidden state from the $(l-1)$-th layer of $m_{i-1}$ is immediately passed to the $l$-th layer of $m_i$ while the forward pass of $m_{i-1}$ is still ongoing (see Figure~\ref{fig:inference}).
For implementation, we maintain a thread-safe shared hidden state pool $g$ for inter-model communication. At each decoding step $t$ and each layer $l$, model $m_i$ waits for the corresponding hidden state $h^{(i-1)}_{l-1,t}$ from its upstream model $m_{i-1}$. Once $h^{(i-1)}_{l-1,t}$ becomes available, it is pushed into $g$ and immediately consumed by $m_i$ to compute $h^{(i)}_{l,t}$.



Finally, after all $(n+1)$ models complete their forward passes at step $t$, their logits are fused following the Key-Logits Backward Pass rule. The final logits $z_t$ are computed according to Eq.~\ref{equ:logitsFusion}, from which the next token is generated.






==> content/4_analyses.tex <==

\section{Theoretical Guarantees: Why Sequential Correction Works}
\label{sec:analysis}

In the previous section, we introduced \modelname, a framework built on the principle of sequential error correction. A natural and critical question arises: does this boosting-style integration of models guarantee a performance improvement? This section provides a formal theoretical justification covering two key aspects: (1) Inference Efficacy, demonstrating that adding a new model provably reduces prediction error under a validity condition; and (2) Optimization Stability, proving that our dual-objective training guarantees a descent path on the primary task.

Our analysis focuses on the Mean Squared Error (MSE) between the ensemble's predicted probability distribution and the ground truth. We encapsulate the requirement for effective correction in a core assumption. For brevity, we present the main results here; full proofs and detailed derivations are provided in Appendix~\ref{app:proof_of_thm_and_cor}.


\textbf{Notations for Analysis}. At decoding step $t$, let $A_i$ denote the sampling space of $m_i$.
We consider an ensemble $\mathcal{M}_i$ with accumulated logits $\hat{z}^{(i)}_t$, yielding predicted distribution $\hat{P}^{(i)}_t=\mathrm{softmax}(\hat{z}^{(i)}_t)$.
Let $\hat{y}^{(i-1)}_{<t}$ be the sequence generated by $\mathcal{M}_{i-1}$ up to step $t-1$, and let $p^*_t(\cdot \mid X_\tau,\hat{y}^{(i-1)}_{<t})$ denote the ground-truth distribution, represented by the one-hot vector $p^\ast_t$.
The residual error of $\mathcal{M}_{i-1}$ is defined as $e^{(i-1)}_t=p^\ast_t - \hat{P}^{(i-1)}_t$.
  To quantify how a new model $m_i$ influences the ensemble's prediction, we define its effective linear contribution to the probability space as $g^{(i)}_t \triangleq J_{\mathrm{softmax}}(\hat{z}^{(i-1)}_t) z^{(i)}_t$, where $J_{\mathrm{softmax}}(\hat{z}^{(i-1)}_t)$ is the Jacobian matrix of the softmax function evaluated at $\hat{z}^{(i-1)}_t$. 

\subsection{Inference Efficacy: Error Reduction Guarantee}
% inference-version
\begin{assumption}
\label{ass:correction_efficacy}
For any model $i \geq 1$, any decoding step $t$, and any vocabulary dimension $v \in \{1, \dots, |\mathcal{V}|\}$, we assume that the successor model $m_i$ produces an effective linear contribution $g^{(i)}_t$ that is a valid corrective term of the residual error vector $e^{(i-1)}_t$. Specifically, we assume its systematic bias in fitting this residual is less than the total uncertainty of the residual. Formally, given a generated context $(X_\tau, \hat{y}^{(i-1)}_{<t})$:
\begin{equation}
\epsilon_{g^{(i)}_{t, v}} < \sqrt{\epsilon_{i-1, t, v}^2 + \sigma_{i-1, t, v}^2},
\end{equation}
where we let $\Theta_{i-1} := \{\theta_0, \dots, \theta_{i-1}\}$ be the parameters of the ensemble $\mathcal{M}_{i-1}$, drawn from a joint distribution $\mathcal{A}_{i-1}$. The bias ($\epsilon^2$) and variance ($\sigma^2$) terms are defined as:

\begin{align}
% Bias of the preceding ensemble M_{i-1} at inference
\epsilon_{i-1, t, v}^2 &:= \mathbb{E}_{(X_\tau,Y_\tau)\sim\mathcal{D}} \left[ \left( p^*_{t,v} - \mathbb{E}_{\Theta_{i-1} \sim \mathcal{A}_{i-1}}[\hat{P}^{(i-1)}_{t,v} \mid X_\tau, \hat{y}^{(i-1)}_{<t}] \right)^2 \right] < \infty, \\
% Variance of the preceding ensemble M_{i-1} at inference
\sigma_{i-1, t, v}^2 &:= \mathbb{E}_{(X_\tau,Y_\tau)\sim\mathcal{D}} \left[ \mathrm{Var}_{\Theta_{i-1} \sim \mathcal{A}_{i-1}}[\hat{P}^{(i-1)}_{t,v} \mid X_\tau, \hat{y}^{(i-1)}_{<t}] \right] < \infty , \\
% Bias of the new model m_i's contribution h^i_t in fitting the residual at inference
\epsilon_{g^{(i)}_{t, v}}^2 &:= \mathbb{E}_{\substack{\Theta_{i-1} \sim \mathcal{A}_{i-1} \\ (X_\tau,Y_\tau)\sim\mathcal{D}}} \left[ \left( e^{(i-1)}_{t,v} - \mathbb{E}_{\theta_i \sim A_i}[g^{(i)}_{t,v} \mid \Theta_{i-1}, X_\tau, \hat{y}^{(i-1)}_{<t}] \right)^2 \right] < \infty.
\end{align}
Furthermore, we assume that the logits generated by the successor model have a finite fourth moment, i.e., $\mathbb{E}[\|z^{(i)}_t(\cdot \mid X_\tau, \hat{y}^{(i-1)}_{<t})\|_2^4] < \infty$.
\end{assumption}


This assumption posits that each boosting step is productive—the new model is more accurate at predicting the error than the existing ensemble is at predicting the target. Our chain training paradigm is explicitly designed to encourage this condition. Based on this assumption, we establish the following theorem and corollary.

\begin{theorem}
\label{thm:mse_reduction}
Under Assumption \ref{ass:correction_efficacy}, For each model $i \geq 1$, decoding step $t$, and vocabulary dimension $v$, there exists an upper bound $\lambda_{i, t, v}^* > 0$ for the scaling coefficient. For any weight $\lambda_{i} \in (0, \lambda_{i, t, v}^*)$, the expected squared error of the new ensemble $\mathcal{M}_{i}$ at inference is strictly lower than that of the predecessor ensemble $\mathcal{M}_{i-1}$ for that dimension. Specifically:
\begin{equation}
\begin{aligned}
\mathbb{E}_{\substack{\Theta_{i-1} \sim \mathcal{A}_{i-1} \\ \theta_i \sim A_i \\ (X_\tau,Y_\tau)\sim\mathcal{D}}}
\left[ \left( p^*_{t,v} - \hat{P}^{(i)}_{t,v} \right)^2 \mid X_\tau, \hat{y}^{(i-1)}_{<t} \right]
<
\mathbb{E}_{\substack{\Theta_{i-1} \sim \mathcal{A}_{i-1} \\ (X_\tau,Y_\tau)\sim\mathcal{D}}}
\left[ \left( p^*_{t,v} - \hat{P}^{(i-1)}_{t,v} \right)^2 \mid X_\tau, \hat{y}^{(i-1)}_{<t} \right].
\end{aligned}
\end{equation}
\end{theorem}


\subsection{Optimization Stability: Guaranteed Descent}
\label{sec:optimization}

While Theorem~\ref{thm:mse_reduction} guarantees that a valid corrector improves inference performance, it relies on the premise that the model can be effectively trained to act as such a corrector. A potential concern with our dual-objective training (Eq.~\ref{equ:totalloss}) is that the error-suppression loss $\mathcal{L}_{s}$ might conflict with the primary cross-entropy loss $\mathcal{L}_{ce}$, potentially destabilizing the training.
To address this, we analyze the optimization landscape and show that a constructive descent path always exists.

We introduce a geometric assumption regarding the alignment between the primary gradient $g_{ce}$ and the error-suppression gradient $g_{s}$.

\begin{assumption}[Gradient Relative Alignment]
\label{ass:grad_align_short}
We assume the error-suppression gradient does not strictly oppose the primary gradient. Formally, there exist constants $0< \rho_i < 1$ and $\Gamma_i > 0$ such that $\langle g_{s}, g_{ce} \rangle \ge -\rho_i \|g_{s}\| \|g_{ce}\|$ and $\|g_{s}\| \le \Gamma_i \|g_{ce}\|$.
\end{assumption}

This assumption is mild in practice due to the mutual exclusivity of the softmax function (suppressing an error token naturally reallocates probability mass to the ground truth). Based on this, we establish the existence of a valid descent path:

\begin{theorem}[Guaranteed Descent on Primary Loss]
\label{thm:descent_short}
Under Assumption~\ref{ass:grad_align_short} and standard smoothness conditions, there exists a lower bound for the balancing coefficient $\alpha > \rho_i \Gamma_i$ and a corresponding learning rate range $(0, \eta^*(\alpha)]$ such that every gradient update step strictly decreases the primary cross-entropy loss $\mathcal{L}_{ce}$.
\end{theorem}

The detailed proof and constructive derivation of $\eta$ can be found in Appendix~\ref{app:support}.

\vspace{0.5em}
\noindent\textbf{Remark and Interpretation}.
Theorems \ref{thm:mse_reduction} and \ref{thm:descent_short} jointly constitute the theoretical foundation of \modelname. 
First, Theorem \ref{thm:mse_reduction} establishes the efficacy of the ensemble: it guarantees that as long as the new model acts as a valid corrector (bias $<$ uncertainty), the system's accuracy improves. The existence of the bound $\lambda$ reflects the classic bias-variance trade-off, where the ensemble weight must balance the correction signal against introduced variance.
Second, Theorem \ref{thm:descent_short} establishes the learnability of the model: it proves that despite the auxiliary error-suppression objective, a valid optimization path exists where the primary task performance monotonically improves.
Together, these results confirm that \modelname is not only effective in principle but also trainable in practice, setting the stage for the empirical validation in Section~\ref{sec:experiments}.


==> content/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We conduct extensive experiments to evaluate the effectiveness and efficiency of our proposed method. 
First, we evaluate \modelname's performance on two representative tasks, Commonsense Reasoning and Arithmetic Reasoning. 
Second, to verify the generality of our approach, we further evaluate \modelname in an industrial scenario provided by the \textit{\dianxinlab}. 
Third, we evaluate the time efficiency of our near-parallel inference paradigm.
Additional experimental results and ablation studies are included in Appendix \ref{appendix: additionalexperiments}. \\
% \input{iclr2026/tables/main_result} \\
\textbf{Commonsense \& Arithmetic Datasets.} To comprehensively evaluate \modelname, we utilize a broad suite of reasoning tasks: (i) Commonsense reasoning: PIQA \citep{bisk2020piqa}, HellaSwag \citep{zellers2019hellaswag}, WinoGrande \citep{sakaguchi2021winogrande},BoolQ \citep{clark2019boolq}, SIQA \citep{sap2019socialiqa}, and OpenbookQA (OBQA) \citep{mihaylov2018can}.
(ii) Arithmetic reasoning: AQuA \citep{ling2017program},GSM8K \citep{cobbe2021training}, MAWPS \citep{koncel2016mawps}, and SVAMP \citep{patel2021nlp}. More details can be found in Appendix~\ref{appendix:datasets}.  \\
\textbf{\dianxindataset(\dianxindatasetshort).} We construct a dataset from real-world public cloud scenarios in \dianxinlab, targeting the evaluation of AI agents in toolchain scheduling. It assesses whether LLMs can interpret user intentions, plan multi-step toolchains, and execute tool calls under realistic industrial constraints. More details can be found in Appendix~\ref{appendix:datasets}.  \\ 
% Unlike existing benchmarks, our dataset introduces multi-tool dependencies, diverse task categories, and varying complexities, offering a more practical test of robustness, generalizability, and utility in tool orchestration.\\
\textbf{Baselines.} To clearly validate the effectiveness of the proposed method, experiments compare it with three mainstream large model optimization and ensembling approaches, namely VOTE \citep{li2024more}, UNITE \citep{yao2024determine}, and T-copilot \citep{zou2025transformer}. Detailed description of these three baseline methods can be found in Appendix \ref{app:baselines}. \\
% \textbf{Implementation Details.} For \modelname, we employ models from both the LLaMA-3 family (LLaMA-3.2-3B, LLaMA-3.1-8B) and the Qwen-2.5 family (Qwen-2.5-3B, Qwen-2.5-7B) as sub-models.  We further extend the generation function from the Huggingface Transformers library to support distributed, token-level inference acceleration across multiple sub-models. All experiments are conducted on four NVIDIA H800 GPUs. More details can be found in Appendix~\ref{app: implementationDetails}. 
%We adopt representative scales from both families as baselines for \textsc{\modelname} and evaluate the proposed framework on \textbf{LLaMA-3.2-3B, LLaMA-3.1-8B, Qwen-2.5-3B, and Qwen-2.5-7B}.
%, ensuring architectural consistency across ensembles by adopting identical decoder-only structures.
% During training, the AdamW optimizer and a linear learning rate scheduler are utilized.

% \input{iclr2026/tables/Matched-ScaleEnsembles}
\input{iclr2026/tables/arithmetic_result}
\input{iclr2026/tables/commonsense_result}
\input{iclr2026/tables/samemodelsize}
% \input{iclr2026/tables/Weakly-HeterogeneousEnsembles}


\subsection{Main Experiments Results}



\textbf{Performance on arithmetic reasoning datasets.}
Table~\ref{tab:arithmetic_result} summarizes the performance on arithmetic reasoning benchmarksunder LoRA training settings. 
\textsc{\modelname} shows a consistent advantage over competing methods, outperforming voting ensembles by a margin of 3.9\% and surpassing stronger baselines by significant margins. 
The effectiveness of our approach is further evidenced by the scaling analysis, where the ensemble achieves a 6.2\% increase in accuracy compared to the single-model baseline. 
Overall, \textsc{\modelname} proves to be a robust solution for enhancing mathematical reasoning capabilities across different model scales.

\textbf{Performance on commonsense datasets.}
Table~\ref{tab:commonsense_result} summarizes the results on commonsense reasoning tasks under LoRA training settings.
\modelname consistently outperforms both majority voting and the UNITE baseline across all six datasets. 
Most notably, it achieves substantial improvements on WinoGrande, surpassing the best baseline by 6.6\%. 
On average, \modelname improves commonsense reasoning accuracy by 1.7\% over the strongest baseline and 5.9\% over voting methods. 
The performance gains are consistent across different model scales, demonstrating that our sequential boosting framework reliably enhances the commonsense reasoning capabilities of base LLMs.






\begin{figure*}[t]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{iclr2026/pictures/memory_usage.png}
    \caption{Training and inference peak memory usage across different models.}
    \label{fig:memory_usage}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{iclr2026/pictures/latency_vs_token.png}
    \caption{End-to-end latency and per-token generation cost.}
    \label{fig:latency_efficiency}
  \end{subfigure}
  \caption{Overall system efficiency comparison of \modelname and baseline ensemble methods.}
  \label{fig:system_efficiency_figure}
    \vspace{-2em}
\end{figure*}


% \textbf{Time Efficiency Analysis.}
% We evaluate the inference latency of sequential and near-parallel execution strategies under different ensemble sizes, as shown in Figure~\ref{fig:inference_efficiency}. The results show that sequential inference latency increases almost linearly with the number of models, making scaling expensive in a real-world setting. In contrast, our near-parallel execution reduces the total inference cost to 12.1 seconds, achieving a 47\% reduction in latency compared to sequential execution. This demonstrates that near-parallelization enables \modelname to scale multiple models efficiently while maintaining practical inference speed.


\textbf{Efficiency and Cost Analysis.}
We evaluate end-to-end wall-clock time, per-token latency, and peak GPU memory during both training and inference, with results shown in Figure~\ref{fig:system_efficiency_figure}. \modelname (7B+7B, near-parallel, 2 GPUs) achieves an end-to-end latency of 13.75 seconds, significantly outperforming ensemble baselines such as UNITE (22.66 s), VOTE (22.61 s), and T-Copilot (17.21 s), and it remains competitive even when restricted to a single GPU. The per-token latency of \modelname (0.075 s/token) is also lower than that of VOTE (0.127 s/token), UNITE (0.128 s/token), and T-Copilot (0.097 s/token), reflecting improved throughput. In terms of memory usage, \modelname reaches 33.18\% peak training memory and 20.72\% peak inference memory per GPU in the 2-GPU configuration, which is comparable to or below the levels of other ensemble systems. The 1-GPU results follow a similar trend. The cost introduced by cross-model state passing is minimal 0.0009 s on 2 GPUs and 0.0002 s on 1 GPU and has negligible impact on the overall latency. Taken together, these findings show that \modelname achieves a more favorable combination of speed, memory efficiency, and coordination cost than existing ensemble approaches, while still providing strong accuracy gains.
All efficiency measurements were conducted on an NVIDIA H800 GPU cluster using the AQuA dataset, with identical decoding settings across all methods. 
A theoretical analysis of inference-time behavior under different execution strategies is provided in Appendix~\ref{app:inferenceTimeEfficiencyAnalysis}.



\textbf{Comparison under equal parameter budgets.}
We compare \modelname with single-model baselines of equivalent parameter counts under the supervised fine-tuning (SFT) setting. As shown in Table~\ref{tab:main_result}, \modelname built from two Qwen2.5-3B models (6B total) reaches the same level of commonsense performance as the 7B model and achieves a higher arithmetic score, improving the average from 77.5 to 78.0, while using 1B fewer parameters.
Under a 14B budget, \modelname constructed from two Qwen2.5-7B models also shows consistent advantages. On HellaSwag, performance increases from 92.9 to 95.1; on SVAMP, from 87.4 to 88.8; and the overall commonsense average rises from 85.1 to 85.6. Arithmetic reasoning similarly improves from 80.1 to 80.2.
In terms of efficiency, per-token latency decreases from 98 ms to 75 ms, corresponding to a 23\% speedup under the same parameter budget. Overall, \modelname provides both higher accuracy and faster inference than single LLMs with equivalent total size.

\textbf{Weakly Heterogeneous Model Ensemble.} We further evaluate \modelname under a weakly heterogeneous configuration by integrating two models from the same family but belonging to different series. In practice, integrating models from different families is difficult because their tokenizers are incompatible; even within a single family, different parameter sizes may adopt different vocabularies (e.g., Qwen2.5-7B and Qwen2.5-3B). Such tokenizer mismatches lead to inconsistent token boundaries during decoding, preventing \modelname from performing accurate layer-wise residual correction. Based on this, we focus on the compatible model pair of Llama3.1-8B and Llama3.2-3B, which maintain consistency in both tokenizer and architectural specifications.
As shown in Table~\ref{tab:main_result}, the weakly heterogeneous ensemble (8B + 3B) improves the average commonsense score from 80.0 to 83.7 and raises the arithmetic average from 68.2 to 69.1 compared with the stronger 8B model alone. This accuracy gain comes with only a minimal increase in computational cost: the per-token latency rises slightly from 0.038 s to 0.049 s, indicating that the ensemble adds only marginal overhead. These results show that even when combining models of different series and scales, \modelname continues to provide consistent benefits in both accuracy and efficiency. This demonstrates that our boosting framework extends beyond strictly homogeneous ensembles and offers a viable approach for integrating diverse model variants within the same family.



\begin{wraptable}{r}{0.4\textwidth} % 稍微调窄一点宽度
    \vspace{-20pt}
    \centering
    \caption{Performance on CCAD.}
    \label{exp:dianxindataset}
    % 使用 \small 或 \footnotesize 调整基准字体大小
    % 注意：如果用了 resizebox，这里的字体大小影响不大，
    % 建议先去掉 resizebox 或者把表格内容做得更紧凑
    \resizebox{\linewidth}{!}{ 
        \input{iclr2026/tables/dianxindataset}
    }
    \vspace{-10pt}
\end{wraptable}
\textbf{Performance on \dianxindatasetshort.} 
As detailed in Table~\ref{exp:dianxindataset}, \textsc{\modelname} establishes a new state-of-the-art on \dianxindataset, exhibiting remarkable robustness across the Llama and Qwen model families. 
Compared to traditional ensemble strategies like VOTE and UNITE, our approach yields consistent improvements of 3.0\% (Llama-3.1-8B) and 2.5\% (Qwen-2.5-7B), highlighting its ability to effectively aggregate weak learners. 
Crucially, the advantages of \textsc{\modelname} are even more pronounced in deployment settings. 
In large-scale end-to-end toolchain scheduling evaluations conducted at \dianxinlab, our method achieves a significant 5\% gain over existing solutions. 
This result serves as strong evidence of its scalability and practical utility in optimizing complex, industrial-grade production pipelines.

==> content/6_conclusion.tex <==
\section{Conclusion}
% We propose \modelname, a novel ensemble learning framework for LLMs with boosting style. It leverages a cross-model attention to enable subsequent models to use predecessor models’ intermediate hidden states. We further introduce a near-parallel inference paradigm that significantly improves efficiency. Extensive experiments show that \modelname outperforms baselines like VOTE, effectively enhancing the model’s reasoning ability, and significantly accelerating inference efficiency compared to traditional ensembles.More discussions are provided in Appendix \ref{appendix:limitation}
We propose \modelname, a novel boosting-style ensemble learning framework for LLMs. It leverages cross-model attention, enabling subsequent models to utilize the intermediate hidden states of their predecessors. We further introduce a near-parallel inference paradigm that substantially improves efficiency. Extensive experiments demonstrate that \modelname outperforms baselines such as VOTE, effectively enhancing reasoning ability and significantly accelerating inference compared to traditional ensembles. Additional discussions are provided in Appendix \ref{appendix:limitation}.

\textbf{Future work.} In future work, we plan to extend our framework to multi-agent settings, where different agents can specialize in reasoning, planning, or tool usage. We will further explore adaptive routing mechanisms that dynamically select agents or reasoning paths based on task context and system states, enabling faster inference and more efficient resource utilization. Combined with speculative reasoning, such routing is expected to reduce latency and improve scalability in large-scale deployments.



==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/tables/Matched-ScaleEnsembles.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) of SFT-trained models under \textbf{Matched-Scale} settings on arithmetic reasoning tasks. \modelname achieves superior accuracy with reduced latency compared to single-model baselines.}
    \label{tab:sft_matched_arithmetic}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l l c c c c c c c c@{}}
        \toprule
        Model & Params & Latency & AQuA & GSM8K & MAWPS & SVAMP & AIME25 & Math500 & Avg. \\
        \midrule
        Qwen2.5-7B & 7B & 0.056 & 56.7 & 84.5 & 93.6 & 85.1 & 11.1 & 60.5 & 65.2 \\
        \rowcolor{gray!14} 
        \modelname(3B $\times$ 2) & 6B \textcolor{red}{\small(-1B)} & \textbf{0.043} &  &  &  &  &  &  & \textbf{} \\
        \midrule
        Qwen2.5-14B & 14B & 0.098 &  &  &  &  &  &  &  \\
        \rowcolor{gray!14}  
        \modelname(7B $\times$ 2) & 14B & \textbf{0.075} &  &  &  &  &  &  & \textbf{} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> iclr2026/tables/Weakly-HeterogeneousEnsembles.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) of LoRA-trained models under \textbf{Weakly-Heterogeneous} settings. Combining Llama-3.1-8B and Llama-3.2-3B via \modelname results in significant gains in both commonsense and arithmetic reasoning.}
    \label{tab:lora_hetero}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l c c c c c c c l c c c c c l@{}}
        \toprule
        \multirow{2}{*}{Model} & latency & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-9} \cmidrule(l){10-14}
        & (s/token $\downarrow$) & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        LLama-3.2-3B  & 0.027 & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        Llama-3.1-8B  & 0.038 &83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \rowcolor{gray!14} 
        \modelname(8B + 3B) & 0.049 & 85.9 & 85.0 & 93.8 & 71.3 & 80.4 & 84.0 & \textbf{83.7} & 43.7 & 64.4 & 89.7 & 78.6 & \textbf{69.1}  \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> iclr2026/tables/ar70B.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model Performance and Efficiency Comparison}
  \begin{tabular}{lccccccc}
    \toprule
    Model                          & Params & Latency & AQUA  & GSM8K & MAWPS  & SVAMP & Avg   \\
    \midrule
    Llama3.1-70B                   & 70B    & 0.254   & 59.1  & 77.4  & 91.6  & 82.6  & 77.7  \\
    LLMBoost (8B $\times$ 3) & 24B    & 0.064   & 47.6  & 68.5  & 92.0  & 81.3  & 72.4  \\
    LLMBoost (8B $\times$ 1) & 8B     & 0.038  & 42.3  & 63.7  & 89.5  & 77.4  & 68.2  \\ 
    \bottomrule
  \end{tabular}
  \label{tab:ar70B}
\end{table}

==> iclr2026/tables/co70B.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model Performance on Commonsense Reasoning Tasks}
  \begin{tabular}{l@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c}
    \toprule
    Model               & Params & Latency & PIQA  & WinoG & HellaS. & Boolq & SIQA  & OBQA  & Avg   \\
    \midrule
    Llama3.1-70B        & 70B    & 0.254   & 93.2  & 93.1  & 96.9    & 76.5  & 82.4  & 92.0  & 89.2  \\
    LLMBoost (8B×3)     & 24B    & 0.064   & 87.4  & 86.3  & 95.2    & 71.7  & 80.7  & 84.8  & 84.5  \\
    LLMBoost (8B×1)     & 8B     & 0.038   & 83.3  & 81.8  & 90.6    & 69.5  & 75.8  & 79.0  & 80.0  \\
    \bottomrule
  \end{tabular}
  \label{tab:co70B}
\end{table}

==> iclr2026/tables/dataset_template.tex <==
% % \begin{table}[H]
% %     \centering
% %     \small
% %     \caption{Examples of dataset templates used in \modelname.}
% %     \label{tab:dataset_template}
% %     \resizebox{\linewidth}{!}{%
% %     \begin{tabular}{l|p{\linewidth}}
% %     \toprule
% %     \textbf{Task Type} & \textbf{Template} \\
% %     \midrule
% %     \multirow{15}{*}{\textbf{Commonsense Reasoning}}
% %     & \textbf{Input:} Please choose the correct solution to the question: To fight Ivan Drago in Rocky for sega master system.
% %     \newline
% %     Solution1: Drago isn't in this game because it was released before Rocky IV.
% %     \newline
% %     Solution2: You have to defeat Apollo Creed and Clubber Lang first.
% %     \newline
% %     Answer format: solution1/solution2     
% %     \newline \newline 
% %     \textbf{Answer:} the correct answer is solution2. \\
% %     \cmidrule{2-2}
% %     &  \textbf{Input:} Please choose the correct answer to fill in the blank to complete the given sentence: Sarah was a much better surgeon than Maria so () always got the harder cases.
% %     \newline
% %     Option1: Sarah 
% %     \newline
% %     Option2: Maria 
% %     \newline
% %     Answer format: option1/option2
% %     \newline \newline
% %     \textbf{Answer:} the correct answer is option1. \\
% %     \cmidrule{2-2}
% %     &  \textbf{Input:} Please answer the following question with true or false, question: is there a difference between hydroxyzine hcl and hydroxyzine pam?
% %     \newline
% %     Answer format: true/false
% %     \newline \newline
% %     \textbf{Answer:} the correct answer is true. \\
% %     \midrule
% %     \multirow{19}{*}{\textbf{Arithmetic Reasoning}} & 
% %     \textbf{Input:} In a school there are 569 girls and 236 boys. How many more girls than boys does the school have?
% %     \newline \newline 
% %     \textbf{Answer:}  
% %     There are 569 girls and 236 boys. The difference between them is 569 - 236 = 333. The school has 333 more girls than boys. The answer is 333. \\
% %     \cmidrule{2-2}
% %     &  \textbf{Input:} A study reported that in a random sampling of 100 women over the age of 35 , 8 of the women were married 2 or more times . Based on the study results , how many woman in a group of 5000 women over the age of 35 would likely be married 2 or more times ?
% %     \newline \newline
% %     \textbf{Answer:} x=(8.0/100.0)*5000.0\\

% %      \cmidrule{2-2}
% %     &  \textbf{Input:} Twenty kids went out on a school trip. In one of the several activities they participated in, they were divided into two equal groups of girls and boys and then went out for a scavenger hunt of seashells. The boys went out for the search and brought back 60 shells each. If the girls brought an amount equal to the number of shells brought by the boys plus four times as many seashells as the boys, how many seashells were brought by each girl?
% %     \newline \newline
% %     \textbf{Answer:} The boys brought back 60 shells each. That means the girls must have brought an amount equal to the number of shells brought by the boys plus four times as many seashells as the boys. That means the girls must have brought 60 + 4 * 60 = 300 shells each. The answer is 300.\\
    
% %     \midrule
% %     \multirow{19}{*}{\textbf{\dianxindatasetshort}} & 
% %     \textbf{Input:}  cloud agent can use following tools: 
% % \newline (1)\textless name\textgreater QueryCloudServerCount\textless/name\textgreater
% % \textless describe\textgreater can query the number of cloud server under the user's account\textless/describe\textgreater
% % \newline (2)\textless name\textgreater QueryUserQuota\textless/name\textgreater
% % \textless describe\textgreater Query the global upper limit of the number of Elastic Public IPs (EIPs), as well as the upper limits in a specified resource pool, including the upper limit of Virtual Machines (VMs), the upper limit of Virtual Private Clouds (VPCs), the upper limit of the total number of storage disks, and the upper limit of the total capacity (in GB) of storage disks.\textless/describe\textgreater
% % \newline (3)\textless name\textgreater QueryCloudServerInformation\textless/name\textgreater
% % \textless describe\textgreater Query cloud server specifications information by \textless param\textgreater user\_id\textless/param\textgreater and \textless param\textgreater cloud\_server\_id\textless/param\textgreater\textless/describe\textgreater
% % \newline (4)\textless name\textgreater QueryCloudResourceList\textless/name\textgreater
% % \textless describe\textgreater Query the names of all cloud resources by \textless param\textgreater user\_id\textless/param\textgreater\textless/describe\textgreater

% % When  cloud agent receives an inquiry: Can I create 2 more cloud hosts? Which tool is  Cloud Agent most likely to call? Answer Choices:

% %     \newline
% %     (A) QueryCloudServerCount and QueryUserQuota
% %     \newline
% %     (B) QueryUserQuota
% %     \newline
% %     (C) QueryCloudServerCount and QueryCloudServerInformation
% %     \newline
% %     (D) QueryCloudServerInformation and QueryCloudResourceList
% %     \newline \newline
% %     \textbf{Answer:} A. \\
% %     \bottomrule
% %     \end{tabular}}
% % \end{table}
% \begin{table}[H]
%     \centering
%     \small
%     \caption{Examples of dataset templates used in \modelname.}
%     \label{tab:dataset_template}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{l|p{\linewidth}}
%     \toprule
%     \textbf{Task Type} & \textbf{Template} \\
%     \midrule
%     \multirow{15}{*}{\textbf{Commonsense Reasoning}}
%     & \textbf{Input:} Please choose the correct solution to the question: To fight Ivan Drago in Rocky for sega master system.
%     \newline
%     Solution1: Drago isn't in this game because it was released before Rocky IV.
%     \newline
%     Solution2: You have to defeat Apollo Creed and Clubber Lang first.
%     \newline
%     Answer format: solution1/solution2     
%     \par \vspace{1ex} % <--- 修复点：替换了 \newline \newline
%     \textbf{Answer:} the correct answer is solution2. \\
%     \cmidrule{2-2}
%     &  \textbf{Input:} Please choose the correct answer to fill in the blank to complete the given sentence: Sarah was a much better surgeon than Maria so () always got the harder cases.
%     \newline
%     Option1: Sarah 
%     \newline
%     Option2: Maria 
%     \newline
%     Answer format: option1/option2
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:} the correct answer is option1. \\
%     \cmidrule{2-2}
%     &  \textbf{Input:} Please answer the following question with true or false, question: is there a difference between hydroxyzine hcl and hydroxyzine pam?
%     \newline
%     Answer format: true/false
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:} the correct answer is true. \\
%     \midrule
%     \multirow{19}{*}{\textbf{Arithmetic Reasoning}} & 
%     \textbf{Input:} In a school there are 569 girls and 236 boys. How many more girls than boys does the school have?
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:}  
%     There are 569 girls and 236 boys. The difference between them is 569 - 236 = 333. The school has 333 more girls than boys. The answer is 333. \\
%     \cmidrule{2-2}
%     &  \textbf{Input:} A study reported that in a random sampling of 100 women over the age of 35 , 8 of the women were married 2 or more times . Based on the study results , how many woman in a group of 5000 women over the age of 35 would likely be married 2 or more times ?
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:} x=(8.0/100.0)*5000.0\\

%      \cmidrule{2-2}
%     &  \textbf{Input:} Twenty kids went out on a school trip. In one of the several activities they participated in, they were divided into two equal groups of girls and boys and then went out for a scavenger hunt of seashells. The boys went out for the search and brought back 60 shells each. If the girls brought an amount equal to the number of shells brought by the boys plus four times as many seashells as the boys, how many seashells were brought by each girl?
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:} The boys brought back 60 shells each. That means the girls must have brought an amount equal to the number of shells brought by the boys plus four times as many seashells as the boys. That means the girls must have brought 60 + 4 * 60 = 300 shells each. The answer is 300.\\
    
%     \midrule
%     \multirow{18}{*}{\textbf{\dianxindatasetshort}} & 
%     \textbf{Input:}  cloud agent can use following tools: 
% \newline (1)\textless name\textgreater QueryCloudServerCount\textless/name\textgreater
% \textless describe\textgreater can query the number of cloud server under the user's account\textless/describe\textgreater
% \newline (2)\textless name\textgreater QueryUserQuota\textless/name\textgreater
% \textless describe\textgreater Query the global upper limit of the number of Elastic Public IPs (EIPs), as well as the upper limits in a specified resource pool, including the upper limit of Virtual Machines (VMs), the upper limit of Virtual Private Clouds (VPCs), the upper limit of the total number of storage disks, and the upper limit of the total capacity (in GB) of storage disks.\textless/describe\textgreater
% \newline (3)\textless name\textgreater QueryCloudServerInformation\textless/name\textgreater
% \textless describe\textgreater Query cloud server specifications information by \textless param\textgreater user\_id\textless/param\textgreater and \textless param\textgreater cloud\_server\_id\textless/param\textgreater\textless/describe\textgreater
% \newline (4)\textless name\textgreater QueryCloudResourceList\textless/name\textgreater
% \textless describe\textgreater Query the names of all cloud resources by \textless param\textgreater user\_id\textless/param\textgreater\textless/describe\textgreater

% When  cloud agent receives an inquiry: Can I create 2 more cloud hosts? Which tool is  Cloud Agent most likely to call? Answer Choices:

%     \newline
%     (A) QueryCloudServerCount and QueryUserQuota
%     \newline
%     (B) QueryUserQuota
%     \newline
%     (C) QueryCloudServerCount and QueryCloudServerInformation
%     \newline
%     (D) QueryCloudServerInformation and QueryCloudResourceList
%     \par \vspace{1ex} % <--- 修复点
%     \textbf{Answer:} A. \\
    
%     \end{tabular}}
    
    
% \end{table}

\begin{table}[H]
    \centering
    \small
    \caption{Examples of dataset templates used in \modelname.}
    \label{tab:dataset_template}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|p{0.9\linewidth}}
    \toprule
    \textbf{Task Type} & \textbf{Template} \\
    \midrule

    \multirow{15}{*}{\textbf{Commonsense Reasoning}} &
    \textbf{Input:} Please choose the correct solution to the question: To fight Ivan Drago in Rocky for sega master system.\par
    Solution1: Drago isn't in this game because it was released before Rocky IV.\par
    Solution2: You have to defeat Apollo Creed and Clubber Lang first.\par
    Answer format: solution1/solution2
    \par\vspace{1ex}
    \textbf{Answer:} the correct answer is solution2. \\
    \cmidrule{2-2}

    &
    \textbf{Input:} Please choose the correct answer to fill in the blank to complete the given sentence: Sarah was a much better surgeon than Maria so () always got the harder cases.\par
    Option1: Sarah\par
    Option2: Maria\par
    Answer format: option1/option2
    \par\vspace{1ex}
    \textbf{Answer:} the correct answer is option1. \\
    \cmidrule{2-2}

    &
    \textbf{Input:} Please answer the following question with true or false: is there a difference between hydroxyzine hcl and hydroxyzine pam?\par
    Answer format: true/false
    \par\vspace{1ex}
    \textbf{Answer:} the correct answer is true. \\
    \midrule

    \multirow{19}{*}{\textbf{Arithmetic Reasoning}} &
    \textbf{Input:} In a school there are 569 girls and 236 boys. How many more girls than boys does the school have?
    \par\vspace{1ex}
    \textbf{Answer:}
    There are 569 girls and 236 boys. The difference between them is $569 - 236 = 333$. The school has 333 more girls than boys. \\
    \cmidrule{2-2}

    &
    \textbf{Input:} A study reported that in a random sampling of 100 women over the age of 35, 8 of the women were married two or more times. Based on the study results, how many women in a group of 5000 women over the age of 35 would likely be married two or more times?
    \par\vspace{1ex}
    \textbf{Answer:} $x = (8/100) \times 5000 = 400$. \\
    \cmidrule{2-2}

    &
    \textbf{Input:} Twenty kids went out on a school trip. They were divided into two equal groups of girls and boys. The boys brought back 60 shells each. If the girls brought the number of shells brought by the boys plus four times as many, how many shells were brought by each girl?
    \par\vspace{1ex}
    \textbf{Answer:} $60 + 4 \times 60 = 300$. The answer is 300. \\
    \midrule

    \multirow{18}{*}{\textbf{\dianxindatasetshort}} &
    \textbf{Input:} Cloud agent can use the following tools:\par
    (1) \textless name\textgreater QueryCloudServerCount\textless/name\textgreater\par
    \textless describe\textgreater query the number of cloud servers under the user's account\textless/describe\textgreater\par
    (2) \textless name\textgreater QueryUserQuota\textless/name\textgreater\par
    \textless describe\textgreater query global and resource pool quotas\textless/describe\textgreater\par
    (3) \textless name\textgreater QueryCloudServerInformation\textless/name\textgreater\par
    \textless describe\textgreater query cloud server specifications\textless/describe\textgreater\par
    (4) \textless name\textgreater QueryCloudResourceList\textless/name\textgreater\par
    \textless describe\textgreater query all cloud resource names\textless/describe\textgreater\par

    When the cloud agent receives an inquiry: \emph{Can I create 2 more cloud hosts?} Which tool is most likely to be called?\par
    (A) QueryCloudServerCount and QueryUserQuota\par
    (B) QueryUserQuota\par
    (C) QueryCloudServerCount and QueryCloudServerInformation\par
    (D) QueryCloudServerInformation and QueryCloudResourceList
    \par\vspace{1ex}
    \textbf{Answer:} A. \\
    \bottomrule

    \end{tabular}}
\end{table}


==> iclr2026/tables/glue.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance of different models on 4 core GLUE subtasks (\%)}
    \small
    \label{tab:glue}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{l|ccccc}
        \toprule
        Model & CoLA & SST-2 & STS-B & MNLI & Avg. \\
        \midrule
        Qwen2.5-14B & 68.31 & 95.78 & 91.93 & 90.77 & 86.70 \\
        tcopilot (Qwen2.5-7B $\times$ 2) & 68.84 & 67.43 & 91.54 & 90.40 & 79.55 \\
        vote (Qwen2.5-7B $\times$ 2) & 69.03 & 95.99 & 92.10 & 90.64 & 86.94 \\
        unite (Qwen2.5-7B $\times$ 2) & 68.93 & 95.99 & 91.67 & 90.58 & 86.79 \\
        LLMBoost (Qwen2.5-7B $\times$ 2) & 69.13 & 96.22 & 92.08 & 90.96 & 87.10 \\
        \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}

==> iclr2026/tables/hyperparameters.tex <==
\begin{table}[!ht]
    \centering
    \caption{Unified hyperparameter configuration of \modelname for LLaMA-3 and Qwen-2.5 series models on \textbf{Commonsense Reasoning} tasks.}
    \label{tab:hyper_commonsense}
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{l|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Hyperparameters}} & \multicolumn{2}{c}{\textbf{Llama Models}} & \multicolumn{2}{c}{\textbf{Qwen Models}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & LLaMA-3.2-3B & LLaMA-3.1-8B & Qwen-2.5-3B & Qwen-2.5-7B \\

    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{Fine-tuning Configurations}}} \\
    Epochs & 2 & 2 & 2 & 2 \\
    Batch Size & 16 & 16 & 16 & 16 \\
    Micro Batch Size & 4 & 4 & 4 & 4 \\
    Cut Off Length & 256 & 256 & 256 & 256 \\
    Maximum Learning Rate & $2e^{-4}$ & $2e^{-4}$ & $2e^{-4}$ & $2e^{-4}$ \\
    Learning Rate Scheduler & Cosine & Cosine & Cosine & Cosine \\
    Optimizer & AdamW & AdamW & AdamW & AdamW \\
    Warmup Steps & 200 & 200 & 200 & 200 \\
    Weight Decay & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{LoRA Configurations}}} \\
    Rank $r$ & 32 & 32 & 32 & 32 \\
    LoRA Alpha & 64 & 64 & 64 & 64 \\
    LoRA Dropout & 0.05 & 0.05 & 0.05 & 0.05 \\
    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{Inference Configurations}}} \\
    Temperature & \multicolumn{4}{c}{0.1} \\
    Top p & \multicolumn{4}{c}{0.95} \\
    Top k & \multicolumn{4}{c}{40} \\
    Maximum New Tokens & \multicolumn{4}{c}{64} \\
    \bottomrule
    \end{tabular}%
    }
\end{table}


\begin{table}[!ht]
    \centering
    \caption{Unified hyperparameter configuration of \modelname for LLaMA-3 and Qwen-2.5 series models on \textbf{Arithmetic Reasoning} tasks.}
    \label{tab:hyper_arithmetic}
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{l|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Hyperparameters}} & \multicolumn{2}{c}{\textbf{Llama Models}} & \multicolumn{2}{c}{\textbf{Qwen Models}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & LLaMA-3.2-3B & LLaMA-3.1-8B & Qwen-2.5-3B & Qwen-2.5-7B \\
    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{Fine-tuning Configurations}}} \\
    Epochs & 2 & 2 & 2 & 2 \\
    Batch Size & 16 & 16 & 16 & 16 \\
    Micro Batch Size & 4 & 4 & 4 & 4 \\
    Cut Off Length & 256 & 256 & 256 & 256 \\
    Maximum Learning Rate & $2e^{-4}$ & $2e^{-4}$ & $2e^{-4}$ & $2e^{-4}$ \\
    Learning Rate Scheduler & Cosine & Cosine & Cosine & Cosine \\
    Optimizer & AdamW & AdamW & AdamW & AdamW \\
    Warmup Steps & 100 & 100 & 100 & 100 \\
    Weight Decay & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{LoRA Configurations}}} \\
    Rank $r$ & 32 & 32 & 32 & 32 \\
    LoRA Alpha & 64 & 64 & 64 & 64 \\
    LoRA Dropout & 0.05 & 0.05 & 0.05 & 0.05 \\
    \midrule
    \rowcolor{gray!20} \multicolumn{5}{l}{\textit{\textbf{Inference Configurations}}} \\
    Temperature & \multicolumn{4}{c}{0.1} \\
    Top p & \multicolumn{4}{c}{0.95} \\
    Top k & \multicolumn{4}{c}{40} \\
    Maximum New Tokens & \multicolumn{4}{c}{256} \\
    \bottomrule
    \end{tabular}%
    }
\end{table}


==> iclr2026/tables/main_result.tex <==
\begin{table*}[!t]
    \centering
    \caption{Comparison of commonsense and arithmetic reasoning performance under matched parameter scales. Results show that \modelname consistently outperforms competitive baselines across different model families and sizes, highlighting its robustness and effectiveness in improving reasoning accuracy.}
    \label{tab:main_result}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|c|c c c c c c l| c c c c c l@{}}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-9} \cmidrule(l){10-14}
        & & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        % \multicolumn{14}{c}{Llama-3.1-8B} \\
        \midrule
        \textbf{Llama-3.1-8B} & $1\times8B$ & 83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times8B$ & 84.2 & 83.2 & 91.4 & 69.8 & 76.9 & 78.4 & 81.0 & 42.8 & 66.5 & 89.7 &  75.7 & 68.7 \\
        vote & $2\times8B$ & 81.7 & 81.3 & 86.8 & 67.3 & 76.1 & 84.8 & 79.7 & 44.4  & 67.8 & 89.5 & 77.5 & 69.8 \\
        UNITE & $2\times8B$ & 86.9 & 84.9 & 93.5 & 70.5 & 79.2 & 84.8 & 83.3 & 42.8 & 65.5 & 89.3 & 76.5 & 68.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times8B$  & 87.9 & 86.1 & 94.5 & 71.7 & 81.6 & 85.6 & \underline{84.4} & 46.8 & 68.8 & 90.1 & 80.1 & \underline{71.5} \\
        \cmidrule(lr){1-14}
        vote & $3\times8B$ & 87.7 & 83.2 & 90.3 & 71.8 & 80.4 & 85.4 & 83.1 & 43.9 & 66.0 &  90.7 & 78.1 & 69.7 \\
        UNITE & $3\times8B$ & 85.3 & 85.0 & 92.2& 70.9 & 79.9 & 85.0 & 83.1 & 43.3 & 65.6 & 88.3 & 77.2 & 68.6 \\
        \rowcolor{gray!14} 
        \modelname & $3\times8B$  & 87.4 & 86.3 & 95.2 & 72.5 & 80.7 & 84.8 & \textbf{84.5} & 47.6 & 68.5 & 92.0 & 81.3 & \textbf{72.4} \\

        \midrule
        \midrule
        % \multicolumn{14}{c}{\textbf{LLama-3.2-3B}} \\
        % \midrule
        \textbf{LLama-3.2-3B} & $1\times3B$ & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times3B$ & 75.7 & 75.9 & 83.4 & 64.6 & 73.8 & 77.2 & 75.1 & 33.3 & 49.5 & 84.6 & 66.7 & 58.5\\
        vote & $2\times3B$ & 79.4 & 76.9 & 84.7 & 66.2 & 75.4 & 75.8 & 76.4 & 34.6 & 50.9 & 85.4 & 68.2 & 59.8 \\
        UNITE & $2\times3B$ & 82.8 & 80.0 & 88.7 & 66.5 & 76.7 & 77.4 & 78.7 & 31.1 & 50.9 & 85.2 & 65.7 & 58.2 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$  & 84.7 & 81.4 & 90.4 & 67.1 & 78.0 & 78.8 & \underline{80.1} & 35.8 & 51.5 & 87.4 & 70.1 & \underline{61.2} \\
        \cmidrule(lr){1-14}
        vote & $3\times3B$ & 80.5 & 76.4 & 85.1 & 66.7 & 77.5 & 77.2 & 77.2 & 32.9 & 53.5 & 87.4 & 66.4 & 60.1 \\
        UNITE & $3\times3B$ & 82.8 & 81.3 & 89.9 & 67.1 & 78.4 & 78.2 & 79.6 & 32.5 & 52.9 & 86.0 & 66.0 & 59.4 \\
        \rowcolor{gray!14} 
        \modelname & $3\times3B$  & 84.2 & 82.0 & 91.5 & 70.2 & 79.0 & 79.6 & \textbf{81.1} & 35.1 & 54.3 & 86.2 & 69.9 & \textbf{61.4} \\

        \midrule[0.35pt]  \midrule[0.35pt]

        % \multicolumn{14}{c}{\textbf{Qwen-2.5-7B}} \\
        % \midrule
        \textbf{Qwen-2.5-7B} & $1\times7B$ & 86.7 & 83.9 & 89.4 & 68.7 & 77.6 & 87.4 & 82.3 & 56.8 & 75.1 & 92.0 & 86.1 & 77.5 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times7B$ & 87.1 & 84.3 & 90.2 & 70.8 & 79.3 & 89.2 & 83.5 & 56.9 & 75.6 & 92.7 & 85.3 & 77.6 \\
        vote & $2\times7B$ & 86.3 & 84.5 & 91.3 & 70.7 & 80.0 & 88.8 & 83.6 & 57.8 & 76.3 & 91.6 & 86.4 & 78.0 \\
        UNITE & $2\times7B$ & 86.1 & 84.1 & 91.6 & 68.6 & 79.1 & 88.2 & 83.0 & 59.5 & 76.3 & 92.2 & 86.4 & 78.6\\
        \rowcolor{gray!18}
        \modelname & $2\times7B$ & 89.5 & 86.7 & 95.1 & 71.6 & 79.1 & 91.6 & \underline{85.6} & 59.8 & 78.1 & 94.1 & 88.8 & \underline{80.2} \\
        \cmidrule(lr){1-14}
        vote & $3\times7B$ & 87.5 & 82.2 & 91.3 & 70.2 & 79.6 & 85.8 & 82.7 & 60.9 & 77.4 & 92.4 & 86.7 & 79.4 \\
        UNITE & $3\times7B$ & 86.1 & 83.3 & 91.5 & 70.3 & 78.4 & 86.8 & 82.7 & 60.9 & 77.8 & 92.8 & 86.3 & 79.5 \\
        \rowcolor{gray!18}
        \modelname & $3\times7B$ & 89.9 & 88.8 & 95.4 & 74.4 & 81.2 & 91.4 & \textbf{86.9} & 61.8 & 78.9 & 93.3 & 88.4 & \textbf{80.6} \\

        \midrule
        \midrule
        % \multicolumn{14}{c}{\textbf{Qwen-2.5-3B}} \\
        % \midrule
        \textbf{Qwen-2.5-3B} & $1\times3B$ & 84.5 & 80.1 & 80.6 & 68.1 & 77.7 & 84.6 & 79.3 & 54.1 & 69.5 & 89.9 & 83.4 & 74.2 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times3B$ & 83.9 & 80.2 & 82.6 & 68.9 & 78.4 & 86.4 & 80.1 & 53.9 & 72.1 & 90.1 & 82.7 & 74.7 \\
        vote & $2\times3B$ & 83.4 & 80.0 & 86.3 & 68.7 & 77.9 & 84.0 & 80.1 & 54.2 & 71.2 & 89.5 & 82.6 & 74.4  \\
        UNITE & $2\times3B$ & 84.1 & 80.6 & 83.5 & 67.3 & 78.0 & 83.0 & 79.4 & 58.5 & 71.6 & 91.3 & 84.7 & 76.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$ & 85.9 & 81.8 & 91.4 & 69.7 & 79.0 & 86.2 & \underline{82.3} & 60.2 & 74.0 & 92.4 & 85.3 & \underline{78.0} \\
        \cmidrule(lr){1-14}
        % \rowcolor{gray!14} 
        vote & $3\times3B$ & 84.1& 79.7 & 87.6 & 67.8 & 77.4 & 83.8 & 80.4 & 59.7 & 71.9 & 92.1 & 85.2 & 77.2 \\
        UNITE & $3\times3B$ & 84.8 & 80.8 & 85.1 & 66.2 & 77.3 & 86.0 & 80.0 & 59.3 & 71.6 & 92.3 & 86.0 & 77.3 \\
        \rowcolor{gray!18}
        \modelname & $3\times3B$  & 86.1 & 82.0 & 91.7 & 70.4 & 80.0 & 87.6 & \textbf{83.0} & 61.2 & 73.4 & 92.6 & 85.6 & \textbf{78.2} \\
        
        \bottomrule
    \end{tabular}
    }
\vspace{-15pt}
\end{table*}

==> tables/Matched-ScaleEnsembles.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) of SFT-trained models under \textbf{Matched-Scale} settings on arithmetic reasoning tasks. \modelname achieves superior accuracy with reduced latency compared to single-model baselines.}
    \label{tab:sft_matched_arithmetic}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l l c c c c c c c c@{}}
        \toprule
        Model & Params & Latency & AQuA & GSM8K & MAWPS & SVAMP & AIME25 & Math500 & Avg. \\
        \midrule
        Qwen2.5-7B & 7B & 0.056 & 56.7 & 84.5 & 93.6 & 85.1 & 11.1 & 60.5 & 65.2 \\
        \rowcolor{gray!14} 
        \modelname(3B $\times$ 2) & 6B \textcolor{red}{\small(-1B)} & \textbf{0.043} &  &  &  &  &  &  & \textbf{} \\
        \midrule
        Qwen2.5-14B & 14B & 0.098 &  &  &  &  &  &  &  \\
        \rowcolor{gray!14}  
        \modelname(7B $\times$ 2) & 14B & \textbf{0.075} &  &  &  &  &  &  & \textbf{} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/Weakly-HeterogeneousEnsembles.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) of LoRA-trained models under \textbf{Weakly-Heterogeneous} settings. Combining Llama-3.1-8B and Llama-3.2-3B via \modelname results in significant gains in both commonsense and arithmetic reasoning.}
    \label{tab:lora_hetero}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l c c c c c c c l c c c c c l@{}}
        \toprule
        \multirow{2}{*}{Model} & latency & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-9} \cmidrule(l){10-14}
        & (s/token $\downarrow$) & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        LLama-3.2-3B  & 0.027 & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        Llama-3.1-8B  & 0.038 &83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \rowcolor{gray!14} 
        \modelname(8B + 3B) & 0.049 & 85.9 & 85.0 & 93.8 & 71.3 & 80.4 & 84.0 & \textbf{83.7} & 43.7 & 64.4 & 89.7 & 78.6 & \textbf{69.1}  \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/ablation.tex <==
\begin{table}[!ht]
\centering
\caption{Ablation study of key components in Ablation study of key components in \textsc{\modelname}, evaluated on mathematical reasoning benchmarks (, evaluated on mathematical reasoning benchmarks (SVAMP, , MAWPS). ``wo E.S.O.'' removes the Error-Suppression Objective; ``wo C.A.'' disables Cross-Model Attention; ``wo ). ``wo E.S.O.'' removes the Error-Suppression Objective; ``wo C.A.'' disables Cross-Model Attention; ``wo $top$--$k$'' ablates the Key-Token Backward Pass (with '' ablates the Key-Token Backward Pass (with $k=2$). ). \modelname consistently outperforms all variants, validating the contribution of each module. consistently outperforms all variants, validating the contribution of each module.}
\label{exp:ablationStudy}
\begin{tabular}{l|lll}
    \toprule
    MODEL TYPE & MAWPS & SVAMP & Avg.  \\ 
    \midrule
    \multicolumn{4}{c}{\textbf{Qwen-2.5-7B as base model}} \\
    \midrule
    \modelname ($2\times7B$) & 88.8 & 94.1 & 91.5\\ 
    wo E.S.O. & 87.3 & 93.3 & 90.3 \\
    wo C.A. & 87.4 & 92.4 & 89.9 \\
    wo $top$-$k$ & 87.2 & 93.3 & 90.3\\
    \bottomrule
\end{tabular}
\end{table}

==> tables/alpha.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) under different $\alpha$ selections.}
    \small
    \label{tab:alpha}
    \begin{tabular}{l|c|ccc}
        \toprule
        Params & $\alpha$ & SVAMP & MAWPS & Avg. \\
        \midrule
        \multicolumn{5}{c}{\textbf{Qwen-2.5-7B as base model}} \\
        \midrule
        \multirow{5}{*}{$2 \times 7$B}
         & 1.00 & 87.0 & 93.7 & 90.4 \\ 
         & 0.99 & 87.0 & 93.7 & 90.4 \\
         & 0.95 & 88.2 & 93.7 & 91.1 \\
         & 0.90 & \textbf{88.8} & \textbf{94.1} & \textbf{91.5} \\
         & 0.80 & 87.9 & 92.9 & 90.4 \\
         & 0.50 & 87.9 & 92.4 & 90.2 \\
        \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}


==> tables/ar70B.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model Performance and Efficiency Comparison}
  \begin{tabular}{lccccccc}
    \toprule
    Model                          & Params & Latency & AQUA  & GSM8K & MAWPS  & SVAMP & Avg   \\
    \midrule
    Llama3.1-70B                   & 70B    & 0.254   & 59.1  & 77.4  & 91.6  & 82.6  & 77.7  \\
    LLMBoost (8B $\times$ 3) & 24B    & 0.064   & 47.6  & 68.5  & 92.0  & 81.3  & 72.4  \\
    LLMBoost (8B $\times$ 1) & 8B     & 0.038  & 42.3  & 63.7  & 89.5  & 77.4  & 68.2  \\ 
    \bottomrule
  \end{tabular}
  \label{tab:ar70B}
\end{table}

==> tables/arithmetic_result.tex <==
\begin{table*}[!t]
    \centering
    \tiny
    % \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{0.9}
    \caption{Performance comparison on \textbf{Arithmetic Reasoning} tasks . The proposed \modelname demonstrates robust improvements on AQuA, GSM8K, MAWPS, and SVAMP.}
    \label{tab:arithmetic_result}
    \small
    \resizebox{0.65\textwidth}{5.5cm}{
    \begin{tabular}{@{}l|c|c c c c c@{}}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-7}
        & & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        
        % === Llama-3.1-8B ===
        \textbf{Llama-3.1-8B} & $1\times8B$ & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \cmidrule(lr){1-7}
        T-copilot & $2\times8B$ & 42.8 & 66.5 & 89.7 &  75.7 & 68.7 \\
        vote & $2\times8B$ & 44.4  & 67.8 & 89.5 & 77.5 & 69.8 \\
        UNITE & $2\times8B$ & 42.8 & 65.5 & 89.3 & 76.5 & 68.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times8B$ & 46.8 & 68.8 & 90.1 & 80.1 & \underline{71.5} \\
        \cmidrule(lr){1-7}
        vote & $3\times8B$ & 43.9 & 66.0 &  90.7 & 78.1 & 69.7 \\
        UNITE & $3\times8B$ & 43.3 & 65.6 & 88.3 & 77.2 & 68.6 \\
        \rowcolor{gray!14} 
        \modelname & $3\times8B$ & 47.6 & 68.5 & 92.0 & 81.3 & \textbf{72.4} \\

        \midrule
        \midrule
        
        % === Llama-3.2-3B ===
        \textbf{LLama-3.2-3B} & $1\times3B$ & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        \cmidrule(lr){1-7}
        T-copilot & $2\times3B$ & 33.3 & 49.5 & 84.6 & 66.7 & 58.5\\
        vote & $2\times3B$ & 34.6 & 50.9 & 85.4 & 68.2 & 59.8 \\
        UNITE & $2\times3B$ & 31.1 & 50.9 & 85.2 & 65.7 & 58.2 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$ & 35.8 & 51.5 & 87.4 & 70.1 & \underline{61.2} \\
        \cmidrule(lr){1-7}
        vote & $3\times3B$ & 32.9 & 53.5 & 87.4 & 66.4 & 60.1 \\
        UNITE & $3\times3B$ & 32.5 & 52.9 & 86.0 & 66.0 & 59.4 \\
        \rowcolor{gray!14} 
        \modelname & $3\times3B$ & 35.1 & 54.3 & 86.2 & 69.9 & \textbf{61.4} \\

        \midrule
        \midrule
        
        % === Qwen-2.5-7B ===
        \textbf{Qwen-2.5-7B} & $1\times7B$ & 56.8 & 75.1 & 92.0 & 86.1 & 77.5 \\
        \cmidrule(lr){1-7}
        T-copilot & $2\times7B$ & 56.9 & 75.6 & 92.7 & 85.3 & 77.6 \\
        vote & $2\times7B$ & 57.8 & 76.3 & 91.6 & 86.4 & 78.0 \\
        UNITE & $2\times7B$ & 59.5 & 76.3 & 92.2 & 86.4 & 78.6\\
        \rowcolor{gray!18}
        \modelname & $2\times7B$ & 59.8 & 78.1 & 94.1 & 88.8 & \underline{80.2} \\
        \cmidrule(lr){1-7}
        vote & $3\times7B$ & 60.9 & 77.4 & 92.4 & 86.7 & 79.4 \\
        UNITE & $3\times7B$ & 60.9 & 77.8 & 92.8 & 86.3 & 79.5 \\
        \rowcolor{gray!18}
        \modelname & $3\times7B$ & 61.8 & 78.9 & 93.3 & 88.4 & \textbf{80.6} \\

        \midrule
        \midrule
        
        % === Qwen-2.5-3B ===
        \textbf{Qwen-2.5-3B} & $1\times3B$ & 54.1 & 69.5 & 89.9 & 83.4 & 74.2 \\
        \cmidrule(lr){1-7}
        T-copilot & $2\times3B$ & 53.9 & 72.1 & 90.1 & 82.7 & 74.7 \\
        vote & $2\times3B$ & 54.2 & 71.2 & 89.5 & 82.6 & 74.4  \\
        UNITE & $2\times3B$ & 58.5 & 71.6 & 91.3 & 84.7 & 76.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$ & 60.2 & 74.0 & 92.4 & 85.3 & \underline{78.0} \\
        \cmidrule(lr){1-7}
        vote & $3\times3B$ & 59.7 & 71.9 & 92.1 & 85.2 & 77.2 \\
        UNITE & $3\times3B$ & 59.3 & 71.6 & 92.3 & 86.0 & 77.3 \\
        \rowcolor{gray!18}
        \modelname & $3\times3B$ & 61.2 & 73.4 & 92.6 & 85.6 & \textbf{78.2} \\
        
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/beta.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) under different $\beta$ selections.}
    \small
    \label{tab:beta}
    \begin{tabular}{l|c|ccc}
        \toprule
        Params & $\beta$ & SVAMP & MAWPS & Avg. \\
        \midrule
        \multicolumn{5}{c}{\textbf{Qwen-2.5-7B as base model}} \\
        \midrule
        \multirow{5}{*}{$2 \times 7$B}
         & 0.01 & 87.0 & 92.4 & 89.7 \\
         & 0.05 & 88.1 & 93.7 & 90.9 \\
         & 0.10 & 88.8 & 92.4 & \textbf{91.5} \\
         & 0.20 & 89.0 & 92.4 & 90.7 \\
         & 0.50 & 88.5 & 92.4 & 90.5 \\
        \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}



==> tables/co70B.tex <==
\begin{table}[htbp]
  \centering
  \caption{Model Performance on Commonsense Reasoning Tasks}
  \begin{tabular}{l@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c}
    \toprule
    Model               & Params & Latency & PIQA  & WinoG & HellaS. & Boolq & SIQA  & OBQA  & Avg   \\
    \midrule
    Llama3.1-70B        & 70B    & 0.254   & 93.2  & 93.1  & 96.9    & 76.5  & 82.4  & 92.0  & 89.2  \\
    LLMBoost (8B×3)     & 24B    & 0.064   & 87.4  & 86.3  & 95.2    & 71.7  & 80.7  & 84.8  & 84.5  \\
    LLMBoost (8B×1)     & 8B     & 0.038   & 83.3  & 81.8  & 90.6    & 69.5  & 75.8  & 79.0  & 80.0  \\
    \bottomrule
  \end{tabular}
  \label{tab:co70B}
\end{table}

==> tables/commonsense_result.tex <==
\begin{table*}[!t]
    \centering
    \scriptsize
    % \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{0.9}
    \caption{Performance comparison on \textbf{Commonsense Reasoning} tasks . \modelname consistently achieves higher accuracy across PIQA, WinoGrande, HellaSwag, BoolQ, SIQA, and OBQA compared to baselines.}
    \label{tab:commonsense_result}
    \small
    \resizebox{0.75\textwidth}{5.5cm}{
    \begin{tabular}{@{}l|c|c c c c c c c@{}}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-9} 
        & & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. \\
        \midrule[0.35pt]
        
        % === Llama-3.1-8B ===
        \textbf{Llama-3.1-8B} & $1\times8B$ & 83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 \\
        \cmidrule(lr){1-9}
        T-copilot & $2\times8B$ & 84.2 & 83.2 & 91.4 & 69.8 & 76.9 & 78.4 & 81.0 \\
        vote & $2\times8B$ & 81.7 & 81.3 & 86.8 & 67.3 & 76.1 & 84.8 & 79.7 \\
        UNITE & $2\times8B$ & 86.9 & 84.9 & 93.5 & 70.5 & 79.2 & 84.8 & 83.3 \\
        \rowcolor{gray!18}
        \modelname & $2\times8B$  & 87.9 & 86.1 & 94.5 & 71.7 & 81.6 & 85.6 & \underline{84.4} \\
        \cmidrule(lr){1-9}
        vote & $3\times8B$ & 87.7 & 83.2 & 90.3 & 71.8 & 80.4 & 85.4 & 83.1 \\
        UNITE & $3\times8B$ & 85.3 & 85.0 & 92.2& 70.9 & 79.9 & 85.0 & 83.1 \\
        \rowcolor{gray!14} 
        \modelname & $3\times8B$  & 87.4 & 86.3 & 95.2 & 72.5 & 80.7 & 84.8 & \textbf{84.5} \\

        \midrule
        \midrule
        
        % === Llama-3.2-3B ===
        \textbf{LLama-3.2-3B} & $1\times3B$ & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 \\
        \cmidrule(lr){1-9}
        T-copilot & $2\times3B$ & 75.7 & 75.9 & 83.4 & 64.6 & 73.8 & 77.2 & 75.1 \\
        vote & $2\times3B$ & 79.4 & 76.9 & 84.7 & 66.2 & 75.4 & 75.8 & 76.4 \\
        UNITE & $2\times3B$ & 82.8 & 80.0 & 88.7 & 66.5 & 76.7 & 77.4 & 78.7 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$  & 84.7 & 81.4 & 90.4 & 67.1 & 78.0 & 78.8 & \underline{80.1} \\
        \cmidrule(lr){1-9}
        vote & $3\times3B$ & 80.5 & 76.4 & 85.1 & 66.7 & 77.5 & 77.2 & 77.2 \\
        UNITE & $3\times3B$ & 82.8 & 81.3 & 89.9 & 67.1 & 78.4 & 78.2 & 79.6 \\
        \rowcolor{gray!14} 
        \modelname & $3\times3B$  & 84.2 & 82.0 & 91.5 & 70.2 & 79.0 & 79.6 & \textbf{81.1} \\

        \midrule
        \midrule

        % === Qwen-2.5-7B ===
        \textbf{Qwen-2.5-7B} & $1\times7B$ & 86.7 & 83.9 & 89.4 & 68.7 & 77.6 & 87.4 & 82.3 \\
        \cmidrule(lr){1-9}
        T-copilot & $2\times7B$ & 87.1 & 84.3 & 90.2 & 70.8 & 79.3 & 89.2 & 83.5 \\
        vote & $2\times7B$ & 86.3 & 84.5 & 91.3 & 70.7 & 80.0 & 88.8 & 83.6 \\
        UNITE & $2\times7B$ & 86.1 & 84.1 & 91.6 & 68.6 & 79.1 & 88.2 & 83.0 \\
        \rowcolor{gray!18}
        \modelname & $2\times7B$ & 89.5 & 86.7 & 95.1 & 71.6 & 79.1 & 91.6 & \underline{85.6} \\
        \cmidrule(lr){1-9}
        vote & $3\times7B$ & 87.5 & 82.2 & 91.3 & 70.2 & 79.6 & 85.8 & 82.7 \\
        UNITE & $3\times7B$ & 86.1 & 83.3 & 91.5 & 70.3 & 78.4 & 86.8 & 82.7 \\
        \rowcolor{gray!18}
        \modelname & $3\times7B$ & 89.9 & 88.8 & 95.4 & 74.4 & 81.2 & 91.4 & \textbf{86.9} \\

        \midrule
        \midrule
        
        % === Qwen-2.5-3B ===
        \textbf{Qwen-2.5-3B} & $1\times3B$ & 84.5 & 80.1 & 80.6 & 68.1 & 77.7 & 84.6 & 79.3 \\
        \cmidrule(lr){1-9}
        T-copilot & $2\times3B$ & 83.9 & 80.2 & 82.6 & 68.9 & 78.4 & 86.4 & 80.1 \\
        vote & $2\times3B$ & 83.4 & 80.0 & 86.3 & 68.7 & 77.9 & 84.0 & 80.1 \\
        UNITE & $2\times3B$ & 84.1 & 80.6 & 83.5 & 67.3 & 78.0 & 83.0 & 79.4 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$ & 85.9 & 81.8 & 91.4 & 69.7 & 79.0 & 86.2 & \underline{82.3} \\
        \cmidrule(lr){1-9}
        vote & $3\times3B$ & 84.1& 79.7 & 87.6 & 67.8 & 77.4 & 83.8 & 80.4 \\
        UNITE & $3\times3B$ & 84.8 & 80.8 & 85.1 & 66.2 & 77.3 & 86.0 & 80.0 \\
        \rowcolor{gray!18}
        \modelname & $3\times3B$  & 86.1 & 82.0 & 91.7 & 70.4 & 80.0 & 87.6 & \textbf{83.0} \\
        
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/dianxindataset.tex <==
% \begin{table}[H] % H = 强制当前位置 (需要 \usepackage{float})
% \caption{Accuracy (\%) on \dianxindataset.}
% \label{exp:dianxindataset}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|l}
%     \toprule
%     Model & Params & \dianxindatasetshort   \\ 
%     \midrule
%     \multicolumn{3}{c}{\textbf{Llama-3.1-8B}} \\
%     \midrule
%     Llama & $1\times8B$ & 52.0\\
%     VOTE & $2\times8B$ & 53.0\\ 
%     UNITE & $2\times8B$ & 52.5\\ 
%     \modelname & $2\times8B$ & \textbf{55.0}\\
%     \midrule
%     \multicolumn{3}{c}{\textbf{Qwen-2.5-7B}} \\
%     \midrule
%     Qwen & $1\times7B$ & 41.0 \\
%     VOTE & $2\times7B$ &  43.0 \\ 
%     UNITE & $2\times7B$ & 41.5 \\ 
%     \modelname & $2\times7B$ & \textbf{45.5}\\
%     \bottomrule
% \end{tabular}
% }

% \end{table}

\begin{tabular}{@{}l c c@{}} % @{} 去除左右多余留白，lcc 表示左对齐、居中、居中
    \toprule
    Model & Params & Acc. (\%) \\ 
    \midrule
    \multicolumn{3}{c}{\textit{Llama-3.1-8B Base}} \\
    \midrule
    Single & 8B & 52.0 \\
    VOTE & $2\times8B$ & 53.0 \\ 
    UNITE & $2\times8B$ & 52.5 \\ 
    \rowcolor{gray!14} % 添加浅灰色背景突出你的模型
    \modelname & $2\times8B$ & \textbf{55.0} \\
    \midrule
    \midrule
    \multicolumn{3}{c}{\textit{Qwen-2.5-7B Base}} \\
    \midrule
    Single & 7B & 41.0 \\
    VOTE & $2\times7B$ & 43.0 \\ 
    UNITE & $2\times7B$ & 41.5 \\ 
    \rowcolor{gray!14}
    \modelname & $2\times7B$ & \textbf{45.5} \\
    \bottomrule
\end{tabular}

==> tables/efficient.tex <==
% 需在导言区加载 booktabs 宏包（\usepackage{booktabs}）
\begin{table*}[!t]
    \centering
    \caption{Efficiency Comparison of Different Models (Time/Memory Metrics)}
    \small
    \label{tab:efficiency}
    \setlength{\tabcolsep}{4pt} % 缩小列间距，平衡紧凑性
    \begin{tabular}{lcccc}
        \toprule
        Model & \makecell{End-to-End\\(s)} & \makecell{Token Cost\\(s)} & \makecell{Peak Train Mem\\(\%)} & \makecell{Peak Infer Mem\\(\%)} \\
        \midrule
        Qwen14B                             & 17.40 & 0.098 & 56.74\% & 36.97\% \\
        LLMBoost 7B+7B (near-par, 2 GPUs)   & 13.75 & 0.075 & 33.18\% & 20.72\% \\
        LLMBoost 7B+7B (near-par, 1 GPU)    & 14.87 & 0.081 & 54.11\% & 39.75\% \\
        LLMBoost 7B+7B+7B (near-par, 3 GPUs)& 18.88 & 0.103 & 33.18\% & 20.13\% \\
        LLMBoost 7B+7B+7B (near-par, 1 GPU) & 21.67 & 0.118 & 73.42\% & 58.48\% \\
        LLMBoost 7B+7B (seq)                & 22.53 & 0.125 & 60.29\% & 38.72\% \\
        VOTE (7B+7B)                        & 22.61 & 0.127 & 53.39\% & 39.14\% \\
        T-Copilot (7B+7B)                   & 17.21 & 0.097 & 64.41\% & 42.05\% \\
        UNITE (7B+7B)                       & 22.66 & 0.128 & 53.39\% & 39.12\% \\
        \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}

==> tables/glue.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance of different models on 4 core GLUE subtasks (\%)}
    \small
    \label{tab:glue}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{l|ccccc}
        \toprule
        Model & CoLA & SST-2 & STS-B & MNLI & Avg. \\
        \midrule
        Qwen2.5-14B & 68.31 & 95.78 & 91.93 & 90.77 & 86.70 \\
        tcopilot (Qwen2.5-7B $\times$ 2) & 68.84 & 67.43 & 91.54 & 90.40 & 79.55 \\
        vote (Qwen2.5-7B $\times$ 2) & 69.03 & 95.99 & 92.10 & 90.64 & 86.94 \\
        unite (Qwen2.5-7B $\times$ 2) & 68.93 & 95.99 & 91.67 & 90.58 & 86.79 \\
        LLMBoost (Qwen2.5-7B $\times$ 2) & 69.13 & 96.22 & 92.08 & 90.96 & 87.10 \\
        \bottomrule
    \end{tabular}
    \vspace{-10pt}
\end{table*}

==> tables/lambdaChoice.tex <==
\begin{table}
\centering
\caption{Sensitivity analysis of the weighting coefficient(s) $\lambda$ in \modelname. Performance (\%) is evaluated across arithmetic reasoning benchmarks (AQuA, MAWPS, SVAMP) under matched parameter scales. The upper block explores $\lambda_1 \in [0.1, 1.0]$ for the \modelname ($2 \times 8B$), while the lower block studies combinations of $\lambda_1, \lambda_2$ for the \modelname ($3 \times 8B$).}
\label{exp:lambdaChoice}
\begin{tabular}{l|c|c c c c}
    \toprule
    Params & $\lambda$ & AQuA & MAWPS & SVAMP & Avg. \\ 
    \midrule
    \multicolumn{6}{c}{\textbf{Llama-3.1-8B as base model}}\\
    \midrule
    \multirow{10}{*}{$2 \times 8B$}
    & 0.1 & 45.7 & 89.4 & 78.9 & 71.3 \\ 
    & 0.2 & 46.4 & 90.1 & 80.0 & 72.2 \\ 
    & 0.3 & 46.8 & 90.1 & 80.1 & \textbf{72.3} \\
    & 0.4 & 43.9 & 90.1 & 80.1 & 71.4 \\ 
    & 0.5 & 46.3 & 89.3 & 79.8 & 71.8 \\ 
    & 0.6 & 46.1 & 90.3 & 79.6 & 72.0 \\
    & 0.7 & 43.9 & 89.7 & 80.0 & 71.2 \\ 
    & 0.8 & 45.3 & 90.7 & 79.9 & 72.0 \\ 
    & 0.9 & 45.7 & 89.9 & 79.5 & 71.7 \\
    & 1.0 & 45.6 & 89.8 & 79.2 & 71.5 \\
    \midrule
    \multirow{3}{*}{$3 \times 8B$}
    & 0.3, 0.1 & 46.9 & 90.7 & 80.4 & 72.7 \\ 
    & 0.3, 0.2 & 46.6 & 92.1 & 80.8 & 73.2 \\ 
    & 0.3, 0.3 & 47.6 & 92.0 & 81.3 & \textbf{73.6} \\
    \bottomrule
\end{tabular}
\end{table}


==> tables/layerskip.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (Performance comparison (\%) under different ) under different \textit{sparsity of cross-model connections sparsity of cross-model connections } settings, i.e., varying the interval of inter-layer interactions. settings, i.e., varying the interval of inter-layer interactions.}
    \label{tab:layerSkip}
    \small
    % \resizebox{0.6\textwidth}{!}{ % 宽度缩小一些更紧凑
    \begin{tabular}{l|l|lll}
        \toprule
        Params & $\phi$ & SVAMP & MAWPS  & Avg. \\ 
        \midrule
        \multicolumn{5}{c}{\textbf{Qwen-2.5-7B as base model}} \\
        \midrule
        \multirow{4}{*}{$2 \times 7B$}
         & 1 & 88.4 & 93.3 & 90.9 \\ 
         & 2 & 88.8 & 94.1 & 91.5 \\ 
         & 3 & 88.1 & 93.3 & 90.7 \\ 
         & 4 & 86.8 & 92.9 & 89.9 \\
        \bottomrule
    \end{tabular}
    % }
    \vspace{-10pt}
\end{table*}


==> tables/main_result.tex <==
\begin{table*}[!t]
    \centering
    \caption{Comparison of commonsense and arithmetic reasoning performance under matched parameter scales. Results show that \modelname consistently outperforms competitive baselines across different model families and sizes, highlighting its robustness and effectiveness in improving reasoning accuracy.}
    \label{tab:main_result}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l|c|c c c c c c l| c c c c c l@{}}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){3-9} \cmidrule(l){10-14}
        & & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        % \multicolumn{14}{c}{Llama-3.1-8B} \\
        \midrule
        \textbf{Llama-3.1-8B} & $1\times8B$ & 83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times8B$ & 84.2 & 83.2 & 91.4 & 69.8 & 76.9 & 78.4 & 81.0 & 42.8 & 66.5 & 89.7 &  75.7 & 68.7 \\
        vote & $2\times8B$ & 81.7 & 81.3 & 86.8 & 67.3 & 76.1 & 84.8 & 79.7 & 44.4  & 67.8 & 89.5 & 77.5 & 69.8 \\
        UNITE & $2\times8B$ & 86.9 & 84.9 & 93.5 & 70.5 & 79.2 & 84.8 & 83.3 & 42.8 & 65.5 & 89.3 & 76.5 & 68.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times8B$  & 87.9 & 86.1 & 94.5 & 71.7 & 81.6 & 85.6 & \underline{84.4} & 46.8 & 68.8 & 90.1 & 80.1 & \underline{71.5} \\
        \cmidrule(lr){1-14}
        vote & $3\times8B$ & 87.7 & 83.2 & 90.3 & 71.8 & 80.4 & 85.4 & 83.1 & 43.9 & 66.0 &  90.7 & 78.1 & 69.7 \\
        UNITE & $3\times8B$ & 85.3 & 85.0 & 92.2& 70.9 & 79.9 & 85.0 & 83.1 & 43.3 & 65.6 & 88.3 & 77.2 & 68.6 \\
        \rowcolor{gray!14} 
        \modelname & $3\times8B$  & 87.4 & 86.3 & 95.2 & 72.5 & 80.7 & 84.8 & \textbf{84.5} & 47.6 & 68.5 & 92.0 & 81.3 & \textbf{72.4} \\

        \midrule
        \midrule
        % \multicolumn{14}{c}{\textbf{LLama-3.2-3B}} \\
        % \midrule
        \textbf{LLama-3.2-3B} & $1\times3B$ & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times3B$ & 75.7 & 75.9 & 83.4 & 64.6 & 73.8 & 77.2 & 75.1 & 33.3 & 49.5 & 84.6 & 66.7 & 58.5\\
        vote & $2\times3B$ & 79.4 & 76.9 & 84.7 & 66.2 & 75.4 & 75.8 & 76.4 & 34.6 & 50.9 & 85.4 & 68.2 & 59.8 \\
        UNITE & $2\times3B$ & 82.8 & 80.0 & 88.7 & 66.5 & 76.7 & 77.4 & 78.7 & 31.1 & 50.9 & 85.2 & 65.7 & 58.2 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$  & 84.7 & 81.4 & 90.4 & 67.1 & 78.0 & 78.8 & \underline{80.1} & 35.8 & 51.5 & 87.4 & 70.1 & \underline{61.2} \\
        \cmidrule(lr){1-14}
        vote & $3\times3B$ & 80.5 & 76.4 & 85.1 & 66.7 & 77.5 & 77.2 & 77.2 & 32.9 & 53.5 & 87.4 & 66.4 & 60.1 \\
        UNITE & $3\times3B$ & 82.8 & 81.3 & 89.9 & 67.1 & 78.4 & 78.2 & 79.6 & 32.5 & 52.9 & 86.0 & 66.0 & 59.4 \\
        \rowcolor{gray!14} 
        \modelname & $3\times3B$  & 84.2 & 82.0 & 91.5 & 70.2 & 79.0 & 79.6 & \textbf{81.1} & 35.1 & 54.3 & 86.2 & 69.9 & \textbf{61.4} \\

        \midrule[0.35pt]  \midrule[0.35pt]

        % \multicolumn{14}{c}{\textbf{Qwen-2.5-7B}} \\
        % \midrule
        \textbf{Qwen-2.5-7B} & $1\times7B$ & 86.7 & 83.9 & 89.4 & 68.7 & 77.6 & 87.4 & 82.3 & 56.8 & 75.1 & 92.0 & 86.1 & 77.5 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times7B$ & 87.1 & 84.3 & 90.2 & 70.8 & 79.3 & 89.2 & 83.5 & 56.9 & 75.6 & 92.7 & 85.3 & 77.6 \\
        vote & $2\times7B$ & 86.3 & 84.5 & 91.3 & 70.7 & 80.0 & 88.8 & 83.6 & 57.8 & 76.3 & 91.6 & 86.4 & 78.0 \\
        UNITE & $2\times7B$ & 86.1 & 84.1 & 91.6 & 68.6 & 79.1 & 88.2 & 83.0 & 59.5 & 76.3 & 92.2 & 86.4 & 78.6\\
        \rowcolor{gray!18}
        \modelname & $2\times7B$ & 89.5 & 86.7 & 95.1 & 71.6 & 79.1 & 91.6 & \underline{85.6} & 59.8 & 78.1 & 94.1 & 88.8 & \underline{80.2} \\
        \cmidrule(lr){1-14}
        vote & $3\times7B$ & 87.5 & 82.2 & 91.3 & 70.2 & 79.6 & 85.8 & 82.7 & 60.9 & 77.4 & 92.4 & 86.7 & 79.4 \\
        UNITE & $3\times7B$ & 86.1 & 83.3 & 91.5 & 70.3 & 78.4 & 86.8 & 82.7 & 60.9 & 77.8 & 92.8 & 86.3 & 79.5 \\
        \rowcolor{gray!18}
        \modelname & $3\times7B$ & 89.9 & 88.8 & 95.4 & 74.4 & 81.2 & 91.4 & \textbf{86.9} & 61.8 & 78.9 & 93.3 & 88.4 & \textbf{80.6} \\

        \midrule
        \midrule
        % \multicolumn{14}{c}{\textbf{Qwen-2.5-3B}} \\
        % \midrule
        \textbf{Qwen-2.5-3B} & $1\times3B$ & 84.5 & 80.1 & 80.6 & 68.1 & 77.7 & 84.6 & 79.3 & 54.1 & 69.5 & 89.9 & 83.4 & 74.2 \\
        \cmidrule(lr){1-14}
        T-copilot & $2\times3B$ & 83.9 & 80.2 & 82.6 & 68.9 & 78.4 & 86.4 & 80.1 & 53.9 & 72.1 & 90.1 & 82.7 & 74.7 \\
        vote & $2\times3B$ & 83.4 & 80.0 & 86.3 & 68.7 & 77.9 & 84.0 & 80.1 & 54.2 & 71.2 & 89.5 & 82.6 & 74.4  \\
        UNITE & $2\times3B$ & 84.1 & 80.6 & 83.5 & 67.3 & 78.0 & 83.0 & 79.4 & 58.5 & 71.6 & 91.3 & 84.7 & 76.5 \\
        \rowcolor{gray!18}
        \modelname & $2\times3B$ & 85.9 & 81.8 & 91.4 & 69.7 & 79.0 & 86.2 & \underline{82.3} & 60.2 & 74.0 & 92.4 & 85.3 & \underline{78.0} \\
        \cmidrule(lr){1-14}
        % \rowcolor{gray!14} 
        vote & $3\times3B$ & 84.1& 79.7 & 87.6 & 67.8 & 77.4 & 83.8 & 80.4 & 59.7 & 71.9 & 92.1 & 85.2 & 77.2 \\
        UNITE & $3\times3B$ & 84.8 & 80.8 & 85.1 & 66.2 & 77.3 & 86.0 & 80.0 & 59.3 & 71.6 & 92.3 & 86.0 & 77.3 \\
        \rowcolor{gray!18}
        \modelname & $3\times3B$  & 86.1 & 82.0 & 91.7 & 70.4 & 80.0 & 87.6 & \textbf{83.0} & 61.2 & 73.4 & 92.6 & 85.6 & \textbf{78.2} \\
        
        \bottomrule
    \end{tabular}
    }
\vspace{-15pt}
\end{table*}

==> tables/numberOfModels.tex <==
\begin{table}[H]
    \caption{Accuracy (\%) across different ensemble sizes on the arithmetic reasoning dataset.}
    \label{tab:numberOfEnsembleModels}
    \centering
    \small  
    \begin{tabular}{l|c|cccc|c}
        \toprule
        Model & Params & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule
        \multicolumn{7}{c}{\textbf{Llama-3.1-8B}} \\
        \midrule
        \modelname & $1\times 8\mathrm{B}$ & 42.3 & 63.7 & 89.5 & 77.4 & 68.2 \\
        \modelname & $2\times 8\mathrm{B}$ & 46.8 & 68.8 & 90.1 & 80.1 & 71.5 \\
        \modelname & $3\times 8\mathrm{B}$ & 47.6 & 68.5 & 92.0 & 81.3 & 72.4 \\
        \modelname & $4\times 8\mathrm{B}$ & 47.1 & 69.3 & 92.1 & 80.9 & 72.4 \\
        \midrule
        \multicolumn{7}{c}{\textbf{Qwen2.5-7B}} \\
        \midrule
        \modelname & $1\times 7\mathrm{B}$ & 56.8 & 75.1 & 92.0 & 86.1 & 77.5 \\
        \modelname & $2\times 7\mathrm{B}$ & 59.8 & 78.1 & 94.1 & 88.8 & 80.2 \\
        \modelname & $3\times 7\mathrm{B}$ & 61.8 & 78.9 & 93.2 & 88.4 & 80.6 \\
        \modelname & $4\times 7\mathrm{B}$ & 62.2 & 78.7 & 93.5 & 88.5 & 80.7 \\
        \bottomrule
    \end{tabular}%
    
    \vspace{-10pt}
\end{table}


==> tables/samemodelsize.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%)  across both matched-scale and weakly-heterogeneous ensembles.}
    \label{tab:main_result}
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{@{}l l c c c c c c c l c c c c c l@{}}
        \toprule
        \multirow{2}{*}{Model} & \multirow{2}{*}{Params}& Latency & \multicolumn{7}{c}{Commonsense Reasoning (Acc. $\uparrow$)} & \multicolumn{5}{c}{Arithmetic Reasoning (Acc. $\uparrow$)} \\
        \cmidrule(l){4-10} \cmidrule(l){11-15}
        & & (s/token $\downarrow$) & PIQA & WinoG. & HellaS. & BoolQ & SIQA & OBQA & Avg. & AQuA & GSM8K & MAWPS & SVAMP & Avg. \\
        \midrule[0.35pt]
        Qwen2.5-7B & 7B & 0.056 & 86.7 & 83.9 & 89.4 & 68.7 & 77.6 & 87.4 & 82.3 & 56.8 & 75.1 & 92.0 & 86.1 & 77.5 \\
        \rowcolor{gray!14} \modelname(3B $\times$ 2) & 6B \textcolor{red}{\small(-1B)} & \textbf{0.043} & 85.9 & 81.8 & 91.7 & 70.4 & 80.0 & 86.2 & \textbf{82.3} & 60.2 & 74.0 & 92.4 & 85.3 & \textbf{78.0} \\
        \midrule
        Qwen2.5-14B & 14B & 0.098 & 90.2 & 85.8 & 92.9& 71.2 & 78.9 & 91.4 & 85.1 & 62.2 & 78.5 & 92.4 & 87.4 & 80.1\\
        \rowcolor{gray!14}  \modelname(7B $\times$ 2) & 14B & \textbf{0.075} & 89.5 & 86.7 & 95.1 & 71.6 & 79.1 & 91.6 & \textbf{85.6} & 59.8 & 78.1 & 94.1 & 88.8 & \textbf{80.2} \\

        \midrule[0.35pt]  \midrule[0.35pt]
        \multicolumn{14}{@{}c}{\textbf{\textit{Weakly-Heterogeneous Ensemble}}}\\
        \midrule
        LLama-3.2-3B & 3B & 0.027 & 78.5 & 77.7 & 83.9 & 62.4 & 74.3 & 76.8 & 75.6 & 31.9 & 49.7 & 84.9 & 65.8 & 58.1 \\
        Llama-3.1-8B & 8B & 0.038 &83.3 & 81.8 & 90.6 & 69.5 & 75.8 & 79.0 & 80.0 & 42.3 & 63.7 & 89.5 & 77.4 & 68.2  \\
        \rowcolor{gray!14} \modelname(8B + 3B) & 11B & 0.049 & 85.9 & 85.0 & 93.8 & 71.3 & 80.4 & 84.0 & \textbf{83.7} & 43.7 & 64.4 & 89.7 & 78.6 & \textbf{69.1}  \\
        \bottomrule
        
    \end{tabular}
    }
\vspace{-15pt}
\end{table*}

==> tables/symbols.tex <==
\begin{table}[htbp]
\centering
\caption{LLMBoost Symbols}
\label{tab:llmboost_symbols}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}p{0.9in}p{3.5in}@{}}
\toprule
$\displaystyle v$ & Vocabulary dimension index \\
$\displaystyle A_i$ & The sampling space of the model  The sampling space of the model $m_i$ \\
$\displaystyle \mathcal{A}_i$ & The sampling space of the ensemble model $\mathcal{M}_i$ \\
$\displaystyle \mathcal{D}$ & Training dataset \\
$\displaystyle d_k$ & Dimension of key matrix \\
$\displaystyle e^{(i)}_{t, v}$ & Residual of $\mathcal{M}_i$ at vocab dimension $v$, t-th token \\
$\displaystyle \mathbb{E}$ & Expectation operator \\
$\displaystyle \mathcal{M}_i$ & Ensemble model at stage $i$ \\
$\displaystyle g$ & Global shared pool \\
$\displaystyle h^{i}_{l,t}$ & Hidden state of $i$-th model,layer $l$, step $t$ \\
$\displaystyle g^{(i)}_{t,v}$ & Linear term of the model $m_i$ in Taylor expansion of softmax \\
$\displaystyle K^{i}_{l,t}$ & Key matrix of $i$-th model,layer $l$, step $t$ \\
$\displaystyle \mathcal{L}_i$ & Loss of $i$-th model \\
$\displaystyle \lambda_i$ & Scaling coefficient for logits fusion \\
$\displaystyle M_i$ & Initial untuned base model \\
$\displaystyle \tilde{M}_i$ & $i$-th model after LoRA fine-tuning \\
$\displaystyle \mathcal{M}$ & Set of base models \\
$\displaystyle \text{MSE}$ & Total Mean squared error\\
$\displaystyle p^{(i)}_t$ & Probability distribution of $i$-th model, t-th token \\
$\displaystyle P^{(i)}_t$ & Probability distribution of $\mathcal{M}_i$, t-th token \\
$\displaystyle Q^{i}$ & Query matrix of $i$-th model \\
$\displaystyle \mathcal{V}$ & Vocabulary set \\
$\displaystyle W_Q, W_K, W_V$ & Projection weight matrices \\
$\displaystyle x$ & Input sequence \\
$\displaystyle y^{*}$ & Ground-truth sequence \\
$\displaystyle \hat{y}_t$ & Token generated at step $t$ \\
$\displaystyle z^{(i)}_t$ & Raw logits of $i$-th model, t-th token\\
$\hat{z}^{(i)}_t$ & Accumulated logits for ensemble $\mathcal{M}_{i}$ at t-th token \\
$\displaystyle \texttt{EOS}$ & End-of-sentence token \\
$\displaystyle \phi$ & LoRA configuration\\
$\displaystyle \theta_i$ & Trainable parameters of $i$-th model \\
$\Theta_{i-1}$  & Parameters of the ensemble $\mathcal{M}_{i-1}$ \\
$X_\tau$ & the input sequence\\
$Y_\tau$ &the corresponding target sequence\\
\bottomrule
\end{tabular}
\end{table}

==> tables/topk.tex <==
\begin{table*}[!t]
    \centering
    \caption{Performance comparison (\%) under different top-$k$ selections on logits.}
    \label{tab:logitsTopk}
    \small
    % \resizebox{0.6\textwidth}{!}{ % 宽度缩小一些更紧凑
    \begin{tabular}{l|l|lll}
        \toprule
        Params & k & SVAMP & MAWPS  & Avg. \\ 
        \midrule
        \multicolumn{5}{c}{\textbf{Qwen-2.5-7B as base model}} \\
        \midrule
        \multirow{8}{*}{$2 \times 7B$}
         & 1 & 87.9 & 92.9  & 90.4 \\ 
        ~ & 2 & 88.8 & 94.1  & \textbf{91.2} \\ 
        ~ & 3 & 88.3 & 93.3  & 90.8 \\ 
        ~ & 4 & 87.3 & 93.4  & 90.4 \\
        ~ & 5 & 87.4 & 93.3  & 90.4 \\
        ~ & 6 & 87.1 & 93.3  & 90.2 \\
        ~ & 7 & 87.2 & 93.3  & 90.3 \\
        ~ & 8 & 87.2 & 93.3  & 90.3 \\
        \bottomrule
    \end{tabular}
    % }
    \vspace{-10pt}
\end{table*}


